Efficient Compactions Between Storage Tiers with PrismDB

In recent years, emerging storage hardware technologies have focused on divergent goals: better performance or lower cost-per-bit. Correspondingly, data systems that employ these technologies are typically optimized either to be fast (but expensive) or cheap (but slow). We take a different approach: by architecting a storage engine to natively utilize two tiers of fast and low-cost storage technologies, we can achieve a Pareto-efficient balance between performance and cost-per-bit. This paper presents the design and implementation of PrismDB, a novel key-value store that exploits two extreme ends of the spectrum of modern NVMe storage technologies (3D XPoint and QLC NAND) simultaneously. Our key contribution is how to efficiently migrate and compact data between two different storage tiers. Inspired by the classic cost-benefit analysis of log cleaning, we develop a new algorithm for multi-tiered storage compaction that balances the benefit of reclaiming space for hot objects in fast storage with the cost of compaction I/O in slow storage. Compared to the standard use of RocksDB on flash in datacenters today, PrismDB's average throughput on tiered storage is 3.3$\times$ faster and its read tail latency is 2$\times$ better, using equivalently priced hardware.

==> ack.tex <==
%-------------------------------------------------------------------------------
\section*{Acknowledgments}
%-------------------------------------------------------------------------------

Mark Callaghan
Jianan Lu
Haoyu Li

==> availability.tex <==
%-------------------------------------------------------------------------------
\section*{Availability}
%-------------------------------------------------------------------------------

USENIX program committees give extra points to submissions that are
backed by artifacts that are publicly available. If you made your code
or data available, it's worth mentioning this fact in a dedicated
section.

==> design_copy.tex <==
%-------------------------------------------------------------------------------
\section{\name Design}
\label{sec:design}
%-------------------------------------------------------------------------------

In this section, we introduce \name, a fast key-value store that blends fast and cheap storage tiers. We first describe \name's design and main system components.

\begin{figure}
  \begin{center}
  {\includegraphics[scale=0.60]{figures/prismdb_v2_system.pdf}}
  \end{center}
  \caption{\label{fig:prismdb-sys} PrismDB system diagram.}
\end{figure}

\subsection{Design Overview} 
\label{sec:design-overview}

Figure~\ref{fig:prismdb-sys} depicts the architecture of \name on two-tiered storage (NVM and flash). 
Since NVM is low latency, in order to reduce synchronization on shared data structures, \name employs a partitioned, shared-nothing architecture, where each worker handles a subset of the key space.
This partitioned approach is extended across all storage tiers; \ie each thread handles its own data structures on DRAM, NVM and flash.

\name uses a hybrid data layout, which is optimized both for NVM and flash. 
At a high level, metadata (\eg indices and bloom filters) are stored on DRAM and NVM, in order to enable fast lookups. 
Both DRAM and NVM also store recently-accessed key-value pairs. In order to support fast writes and reduce writes on flash, all newly-written data (including updates) are written to NVM. Therefore, to optimize for fast random writes and in-place updates, the NVM data layout uses unsorted slabs. The data layout on flash
is optimized for sequential write access, which minimizes write amplification, and is therefore based on a sorted log. 

Each partition has a tracker and a mapper component that are stored in DRAM. The tracker is a key popularity tracker that uses the \clock algorithm to store key accesses. The mapper maintains the \clock value distributions and uses those distributions to enforce the placement of objects on storage. It uses a parameter, called the pinning threshold, to determine whether an object is ``popular'' enough for NVM. Each partition runs a background migration thread to free up space on NVM by moving the colder objects to flash while retaining the popular objects on NVM.
Several key ranges are selected for migration based on an efficient key selection mechanism and the candidate range is selected using a novel migration metric.
We now provide more detail on the data structures on DRAM, NVM, flash.

% TODO: MJF Why "red-block" versus anything else?  SShould yo ujust say "b-tree" rather than the specifics?  Why a b-tree vs. something else?
\paragrapha{In-memory data structures.} Objects on NVM are not sorted. Therefore, for fast look-ups, we use a %Red-Black tree based 
B-tree index to locate NVM objects. Since our design needs to support a large database of small objects, an index over all the keys in the database will not fit in memory. Hence, only the index for objects on NVM is stored in memory.
% objects stored in SST files on flash are not indexed in DRAM.
% 512M key database with object size 1KB takes 900MB in filter and index blocks (with 4KB block size, 2B index entry and 10bit/key bloom filter), compared to 10GB for an equivalent database of 64B object size.
Each index entry in the B-tree uses 13~B to store the key and its NVM address (\ie slab ID and the page offset). 
Each partition also stores the clock-based tracker in memory discussed in \ref{sec:tracker}.  Each tracker entry is 9~B and stores the key and \clock information. \name does not use block cache for caching frequently read objects and instead relies on the OS page caching.

\paragrapha{Data layout on NVM.}
All new data is written to NVM, and it also serves as a second-level read cache after DRAM for hot objects.
We use a slab-based data layout for data stored on NVM, since it needs to support fast random inserts and updates of small objects.  
Slab files contain objects of a particular size range (\eg 64--128~B).
Objects of similar size are inserted into available fixed-size slots within the same slab file, along with a metadata header containing version number, key size and value size information.
If an object is deleted, its slot is freed and ready to store new data. 
Similarly, an update that changes the key-value size range requires freeing the current slot and moving the record to a new slot on another slab file. 
An in-place update can take place on the original slot if the object doesn't change its size range. 
Reading the key-value pair requires navigating to the right slab file and slot offset, decoding the metadata header and reading key and value at the right byte offset. 

NVM also stores the index of the objects stored on flash. The reason we decided to store the index on NVM rather than DRAM, is because reading these objects already incurs the cost of going to QLC (\ie hundreds of microseconds), so it would make a negligible difference to store their index in DRAM. 
In addition, by default, we store the bloom filter for objects stored in flash on NVM.
\name uses a bloom filter~\cite{bloomfilter} for each file on flash to prevent issuing expensive read I/Os to QLC for objects not present in the database. We store the bloom filters on NVM rather than flash, because they take up significant space in a small-object database.
The combined size of the flash index and filters can range from 100s of MBs to 10s of GBs, depending on the object size. 
For a small-object database, the flash index and filters can reside entirely on NVM.
%We decided to store them on NVM rather than wasting precious space on DRAM, since a request that already needs
%instead of DRAM (OS page cache). In the case of a request that already needs to access the much slower flash tier, there would be marginal benefit in conducting the index lookup in DRAM compared to NVM. 
  
\paragrapha{Data layout on flash.} Since flash storage is optimized for sequential writes, we use a Sorted String Table (SST) file format (similar to LSM trees~\cite{leveldb,rocksdb}), which are stored in a log for storing objects on flash. 
% AC I think flash only requires sequential writes, it's fine with random reads
Each SST file has an index block that stores an index for all the data blocks in that file, and a filter block that stores the bloom filter for all the objects present in that file. SST files store disjoint key ranges, which makes searching an object fast.
When the percentage of NVM in \name is 10\% or higher, by default we store all the flash data in a single-level log.  When the percentage is lower, \name by can store the flash data in a multi-level log, similar to an LSM tree. This choice is based on the fan-out of objects stored on NVM and flash, and it provides a knob for controlling write amplification on flash.  For example, a uniform workload with 10\% NVM allocation yields a fan-out of 10; that is, a key range in NVM has an overlap in flash that is 10$\times$ its size. Smaller NVM allocations will cause higher write amplification on flash.

\subsection{Lifecycle of a Written Object}
\begin{figure}
  \begin{center}
    {\includegraphics[scale=0.2]{figures/write-lifecycle.pdf}}
  \end{center}
  \caption{\label{fig:write-lifecycle} Lifecycle of a written object in \name.}
\end{figure}

Figure~\ref{fig:write-lifecycle} illustrates the lifecycle of an object written to \name. 
Objects are always written to NVM because writes needs to be persisted (for crash recovery purposes), and random writes on NVM are much faster than flash. 
When NVM's used capacity hits a high watermark (by default 98\%), the partition triggers a background migration job to demote colder objects to flash until it frees up enough space on NVM (by default 95\%).
In the meantime, incoming writes are rate-limited to ensure that NVM does not exceeds its capacity. 
It selects a subset of existing NVM objects, filters hot ones using the mapper, and \emph{demotes} the rest (\ie the colder objects) to flash.  
At the same time, given that \name is already incurring the cost of writing a new SST file, if the migration job finds hot flash objects, it may \emph{promote} them to NVM during the migration and reclaim their space from flash. In read-heavy workloads, where write-triggered migrations are rare, \name may also proactively trigger migrations when it detects that too many hot keys are accessed from flash, with the goal of promoting hot objects to NVM from flash.
Since NVM stores the most recent data, obsolete versions of objects on flash are automatically deleted when merging with new versions migrated from NVM. 
%They can also be explicitly deleted by the client. 

 

\subsection{Popularity Tracking} 
\label{sec:popularity-tracking}

We now discuss in more detail how \name tracks popular keys, and designates them as hot (or not).

\paragrapha{Tracker: lightweight tracking of keys.} 
\label{sec:tracker}
The tracker estimates object read popularity, while incurring a minimal overhead. There is a large body of work on how to track and estimate object popularity~\cite{LHD,RIPQ,mini-caches,SHARDS,lrb}.
However, many of the existing mechanisms require a relatively large amount of data per object (and computation per access), 
in order to track various access statistics (number of prior accesses, frequency, relationships with other objects, etc.)~\cite{LHD, lrb}. 
Given that key-value objects are often small (\eg less than 1~KB~\cite{cliffhanger,nishtala2013scaling,fb2020}), we need to limit the amount of metadata we use for tracking purposes per object, yet maintain an accurate prediction on how ``hot'' the object is, or how likely it is to be read or updated in the near future. 
In addition, supporting a high number of read operations to the database requires a high-performing mechanism for tracking popularity, \ie one that can track millions of small objects at high throughput.% and to evaluate whether it would provide sufficient information to decide which objects to pin. 

\Clock~\cite{clock} is a classic approach to approximate the least recently used (LRU) eviction policy while offering better space efficiency and concurrency~\cite{fan2013memc3,flashield}.
Using a single \clock bit captures recency, while employing multiple \clock
bits can be used to also track frequency. This makes \clock an attractive 
option for estimating key popularity.  
%in order to group more popular keys on faster storage.
% The number of LSM levels is an upper bound for the different popularity tiers. 

\name's tracker uses the multi-bit \clock algorithm for object tracking.
The tracker uses a concurrent hash map that maps keys to their \clock bits.
%That gives sufficient resolution to capture the heterogeneity of storage in the LSM. 
%In particular, keys get hashed to a bucket. If the bucket has chaining and contains more than one key, then the key is compared to the hash tags. By default, we dedicate 1 byte to the \clock bits and 4 bytes to the hash tag.
Each client read operation requires the tracker to update the \clock bits of the object that was read. %Pinning process (described later), uses the key popularity to pin objects to levels and calls Get() on the popular cache. In other systems like Memcached, Get/Set ratio can be imbalanced (30:1) and proposed cache designs~\cite{fan2013memc3} have tried to exploit that imbalance. We don’t observe a noticeable skew in the Get/Set ratio for our cache (TODO: find this ratio for our system). 
%Since setting the \clock bits is on the critical path of reads, the set operation needs to be lightweight.  This leads to several performance optimizations in the tracker. 
Since setting the \clock bits is on the critical path of reads, we design several performance optimizations.

First, in order to save space, the tracker does not store \clock bits of all key-value pairs in the system, only the most recently-read ones.
Second, the tracker is optimized for concurrent key insertions, evictions and lookups. 
Traditional \clock implementations use a doubly-linked list or a circular buffer that contains the \clock bits along with a hash map that contains the mapping from key to \clock bits, which requires that insertion and eviction operations be serialized. In contrast, \name's tracker does not keep a separate buffer from the hash table. Therefore, it does not require any extra synchronization for those operations, and relies on the synchronization provided by the concurrent hash map. %However, this means we may experience collisions, which will cause the tracker to misidentify a key's \clock bits.
%Third, the tracker conducts eviction offline, in a background process, so that when a read causes a new key to be inserted into the tracker and exceed its size, that doesn't trigger eviction of an older key in the critical path. 

% \begin{figure}[!t]
% 	\centering
% % 	\subfloat[]{
% % 	\label{fig:clock-dist}
% % 		\includegraphics[width=0.45\columnwidth]{figures/\clock.pdf}
% % 	}
% 	\subfloat[]{
% 	\label{fig:clock-ycsb}
% 		\includegraphics[width=0.45\columnwidth]{paper/figures/\clock_percents.pdf}
% 	}
% 	\caption{\clock value distributions of \name using the YCSB B workload (Fig.~\ref{fig:clock-dist}). \clock value distribution across all YCSB workloads (Fig.~\ref{fig:clock-ycsb})}
% 	\label{fig:clock}
% \end{figure}

\begin{figure}
    \begin{center}
    {\includegraphics[width=0.50\columnwidth]{figures/clock_percents.pdf}}
    \end{center}
    \caption{Clock value distributions under different workloads.}
    \label{fig:clock}
\end{figure}

% TODO: we are currently using 4byte hash tag per key. Memc3 paper uses just 1byte tag per key. Might be worth checking if 1byte hash improves/worsens performance.

\paragrapha{Mapper: enforcing the pinning threshold.}
Ideally, \name needs a threshold to determine which objects are hot, which we call the \emph{pinning threshold}.
% TODO: MJF Have we really discussed what "the migration job" was previously?  Partially related to my suggestion for a new 4.2 that talks about "life of a written key"
In other words, at each pass of the migration job, \name should pin some percent (\eg 10\%) of the most popular objects that are being tracked by the tracker on faster storage.

However, determining this threshold is not straightforward, since the relative popularity of the object depends on the \clock bit distribution. 
Consider a two-bit \clock, with 3 being most popular and 0 being least popular. If \name wants to enforce a pinning threshold of 10\%, and exactly 10\% of keys have all their \clock bits set to 3, then \name should pin all the items with a \clock value of 3. However, if 50\% of the keys have a \clock value of 3, then \name cannot pin all items a value of 3, otherwise it will exceed the desired pinning threshold. To illustrate, Figure~\ref{fig:clock} shows that the \clock value distributions change as a function of the workload. 
To this end, the mapper is responsible for keeping track of the \clock value distribution, and uses that distribution to enforce the pinning threshold.
%In order to maintain the \clock value distributions, the mapper maintains the aggregate number of keys that have a particular \clock value in an array. 
%The array gets updated during insertion and eviction. During eviction, the tracker keeps count of the \clock values of all the items it decremented and the item it evicted and updates the mapper with the new distribution. It also updates the mapper when a new item is inserted into the hash map.

\paragrapha{Pinning threshold algorithm.}
%With pinned compactions, each key is looked up in the tracker. Depending on the \clock value of the key, the key distribution, and the desired pinning threshold the placer decided whether to pin the key in upper level or to push the key down. 
In order to enforce the pinning threshold, the mapper uses the following algorithm, which is best illustrated with an example. 
Suppose the \clock distribution is similar to the YCSB-B workload depicted in Figure~\ref{fig:clock},
%(after the distribution stabilizes),
where the percentage of keys with a \clock value of 3 is about 10\%, the percentage of those with a value of 2 is 10\%, the ones with a value of 1 is 30\%, and the remaining 50\% have a \clock value of 0. 

Now, suppose the desired threshold is 15\% (\ie the most popular 15\% of items are stored on NVM, and the rest on flash). If the migration job encounters an item with a \clock value of 3, it will always pin it. If it encounters an item with a \clock value
of 2, it will randomly choose whether to keep it or not (in this example, with a probability of 0.5). If it encounters either an item with \clock value of 1 or 0, or an item that is not currently being tracked (recall the tracker does not track all items in the database), that item will be demoted to flash.

To summarize, the mapper satisfies the pinning threshold using the highest-ranked \clock items by descending rank, and if need be, randomly samples objects that belong to the lowest \clock value that is needed to satisfy the threshold.  

\subsection{Migration Trade-off}
\name uses migration between NVM and flash for two functions.
First, \name uses migration to free up space in NVM when it is close to running out of capacity. Second, during migrations, \name demotes cold objects to flash and promotes hot objects to NVM.
%Second, it collaborates with the popularity tracking mechanism to pin popular objects on faster storage. % Second, since migration already involves reading from and writing to flash (which is expensive), we amortize its cost by using it as a mechanism to place popular objects in NVM and less popular objects in flash.
%Similar to compaction in LSMs, migration is a form of garbage collection. 
%In \name, migration plays a central role in achieving the design goals of low read latency and low flash write amplification. Also, inefficient migrations can stall the foreground client operations and degrade the overall system performance. 
%It is the central piece to realize \name's goals of high performance and low cost.
%Below, we describe the desired properties of migration, discuss the challenges we face, and propose an analytical model to design efficient migrations. 
%\subsubsection{Migration Goals}
However, the two functions of migration, garbage collection and data pinning, present a fundamental trade-off.
%Migration plays a central role in achieving the design goals of low read latency and low flash write amplification. However, migration efficiency and 
On one hand, if \name were to migrate objects from NVM to flash without considering their popularity, then NVM will not serve as an effective second-level read cache.
On the other hand, if \name were to pin a high percentage of objects that it encounters, it will take it much longer (and require more CPU) to free up space in NVM. This will not only delay incoming client writes, but also incur higher flash write amplification. This is because the objects in NVM selected to be demoted will have a ``sparser'' key range, and require the migration job to merge the NVM objects with a larger number of SST files on flash.

%If, as a garbage collector, it cannot free enough space in a timely fashion on NVM, incoming clients writes will be delayed or entirely stalled because NVM will run out of  capacity, leading to worse throughput and latency.

%On the other hand, migration involves reading from and writing to flash.
%If it selects some NVM objects that overlap with a lot of SSTables on flash, merging these objects will incur a lot of data rewrites and very high write amplification. 
%For flash devices like QLC which are known to have limited write cycles, such careless practices will quickly wear out flash and deviates from our primary goal of cost-effectiveness.

\iffalse
To align with \name's main goals of high performance and low cost, we detail out three desired properties of an efficient migration. 

\Paragraph{(1) Read Popularity Awareness}
Flash reads can be orders of magnitude slower compared to NVM. Migrating popular objects to flash can result in poor read performance. Thus, migration needs to be read-popularity aware. Migrations in \name use the mapper to check if an object meets the criteria to be pinned on NVM. Only less popular objects are moved to the flash. This ensures that more reads are served from NVM, which translates to lower latency reads.
%Because reads and writes are of orders of magnitude faster on Optane, \name keeps frequently accessed data on Optane, serving as a secondary cache.
%Migration should respect such hot-cold data separation.
%It works together with clock cache to pin popular data on Optane while only migrating colder data to QLC. 
%This ensures that more reads are served from Optane and delivers lower overall read latency.

\Paragraph{(2) Low Write Amplification}
The proper selection of which objects should be migrated down has a significant impact on the write amplification of the flash. To maintain the proper sort order of SST files, when writing objects from NVM to flash,
objects on NVM need to be merge-sorted with their overlapping SST files on flash and then written back as new SST files. So, a naive selection of objects can result in regularly re-writing most of
the files in flash. 
This would be an undesirable result, given that flash devices (especially QLC)
have limited write cycles and tend to wear out quickly if write amplification is high.  
Thus, migrations need to be optimized for low write amplification.

\Paragraph{(3) Garbage Collection Efficiency}
The primary goal of migration is to free up space on NVM for new incoming writes.
% MJF What is "setup overhead" -> sounds super generic.
Each invocation of migration has a cost, including setup overhead and additional CPU and IO cost. 
Slow migrations can stall foreground client operations, 
by utilizing CPU/IO that could otherwise be spent on processing client-facing read and write operations.
% MJF We don't define "garbage collection" before?  Say here what it means?
Thus, migrations need to run quickly and be efficient in terms of garbage collection.

\fi

\subsubsection{Migration Efficiency Metric}

Since data on NVM is organized as individual key-value pairs and unpopular keys can be scattered across the entire key space, there are many possible choices of which cold objects to select for migration. 
%However, spending a long time in searching which cold objects to migrate increases the overall migration time. % and deviates from our goal as an efficient garbage collector. 
Therefore, to reduce the search space, and to clearly bound the flash I/O caused by each migration, \name divides the contiguous NVM key space into smaller key ranges based on existing SST file bounds on flash. 
We define a migration key range, $i$, as the key ranges of $i$ consecutive SST files. 
%This ensures that a migration key range, if selected, will overlap with $i$ SST files on flash.
%This also helps bound the amount of data rewritten back to flash.
The value of $i$ is tunable in \name, and by default is set to 1.
A higher value of $i$ is more suitable for workloads with smaller SST file size or with many popular objects evenly distributed across the global key space.
% Basically, if the number of cold objects in the migration key range is small, then should consider a higher i to widen the migration key range. 

%\begin{figure}[!t]
%	\centering
%	\subfloat[]{
%	\label{fig:mig-design1}
%		\includegraphics[width=0.5\columnwidth]{figures/mig-design1.pdf}
%	}
%	\subfloat[]{
%	\label{fig:mig-design2}
%		\includegraphics[width=0.35\columnwidth]{figures/mig-design2.pdf}
%	}
%	\caption{ Comparison of strawman and the precise-M key range selection metrics with \name along 3 axes: total flash write I/O, CPU utilization and throughput, using YCSB-A with Zipfian 0.8, 100 million 1~KB requests, 8 partitions and 10 cores.}
%	\label{fig:mig-design}
%\end{figure}

\paragrapha{Which key range should we choose?}
%One question that naturally arises is that, out of the finite number of candidate migration key ranges, which one should migration choose.
The strawman approach is to randomly select a migration key range and move its unpopular objects to flash. 
In order to test this approach, we run a simple experiment with YCSB-A on \name. We observe that when $i=1$, the strawman algorithm selects a key range that contains 12K unpopular keys. However, when we exhaustively search over the key ranges, we find that, at every migration, there exists a key range that on average has 35K unpopular keys. Therefore, the strawman scheme is inefficient, since each migration will cause a relatively small number of keys to migrate but still need to rewrite a single SST file on flash. Therefore, it will incur high write amplification.

%However, we find that this scheme performs poorly.% \name performs poorly under such naive migrations. 
%Figure~\ref{fig:mig-design1} shows that random key selection incurs more than 100GB of write IO to flash when running YCSB-A on a 100GB dataset. 
%This is because its random nature makes it possible to select ranges with high popularity density.
%We observe that, while all migration key ranges overlap with a single SST file, the strawman approach selects one that, on average, contains only 12K unpopular keys whereas some other candidates, if were selected, can migrate more than 35K unpopular keys. 
%Therefore, it has to trigger a lot more migrations to free enough space on NVM and inevitably incurs much higher write amplification on flash. 

%More fundamentally, the strawman approach fails because it doesn't know what is a \emph{good} migration key range.
%This demonstrates that naive migrations can easily violate primary design goals of \name in Section \ref{sec:perf}.
%In the next section, we revisit the objective of migrations and investigate what is considered to be a good migration key range. 

\paragrapha{Analytical model.}
To align with our design goals of cost-efficiency and low flash I/O, the goal of our migration policy is to minimize the amount of flash write I/O per migrated byte. 
During migration, older versions of objects on flash will be deleted when merging with more recent NVM data.
Thus, migrating an NVM key range involves writing its unpopular keys and non-overlapping SST file keys back to flash.
%For workloads with constant object size, this is equivalent to minimizing flash write I/O per migrated key, which equals to the total number of keys re-written to flash divided by the number of migrated keys.
%The write cost per migrated key becomes the total number of keys re-written to flash divided by the number of migrated keys.

We develop an analytical model for object migration cost. 
For simplicity, we initially assume object sizes are equal, and defines notations in terms of ``number of keys'', which directly equates to their size. %For variable-sized objects, these notations can simply be normalized to ``number of bytes''. 
Table~\ref{tab:notation} summarizes the notations and their meanings.
Given an NVM key range, where $p$ is the ratio of popular keys, the number of unpopular keys is \((1-p) \cdot t_{n}\), where $t_{n}$ is the number of keys in a candidate NVM key range.
Meanwhile, $o$ is the fraction of keys in the SST file, that also appear in the NVM key range. Therefore, the number of non-overlapping keys in the SST file is \((1-o) \cdot t_{f}\), where $t_{f}$ is the total number of keys in the original SST file. 

Therefore, the write I/O per migrated key is: \(\frac{(1-o) \cdot t_{f}}{(1-p) \cdot t_{n}}\). We define \(\frac{t_{f}}{t_{n}}\) as the fanout, $F$, which represents the size ratio of key ranges on NVM and flash.
Therefore, the flash I/O cost is reduced to \(F \cdot \frac{ (1-o)}{(1-p)}\).
We define our migration metric, $M$, as the inverse of this cost, where a higher score is better (less write I/O per key):

\vspace{-1em}
\begin{equation}
    M = \frac{1 - p}{F(1 - o)}
    \label{eq:migration}
\end{equation}

For workloads with variable-sized objects, $p$, $o$ and $F$ are normalized by size (in bytes) to compute $M$ precisely.


\begin{table}[t!]
    \centering
    \footnotesize
    % \begin{tabular}{l{0.2cm}l{1.2cm}l{0.2cm}}
    \begin{tabular}{p{0.6cm} p{6.9cm} }
      \toprule 
       Symbol & Description\\
       \midrule
       $p$ & Fraction of popular keys in candidate NVM key range.\\ % It is $\in$ [0,1]. \\
        $\; t_{n}$ & Number of total keys in selected NVM key range. \\
        %\hline
        $o$ & Fraction of overlapping keys between NVM range and flash.\\% It is $\in$ [0,1]. \\
        $\; t_{f}$ & Number of total keys in SST file before merging.  \\
       %\hline
       %$u_{n}$ & Number of unpopular keys in selected NVM key range. \\

       $F$ & The ratio $\frac{t_{f}}{t_{n}}$ between key range on flash and NVM.\\% It equals to \(\frac{Y}{X}\).\\

       \bottomrule
    \end{tabular}
    \caption{Notations}
    \label{tab:notation}
\end{table}

\paragrapha{Precisely computing the migration metric.}
 %and whether we have met our migration objective. 
To test this metric, we first implement a policy that precisely scores candidate key ranges and selects the one with highest value of $M$.
We repeat the same experiment as before with YCSB-A. % to evaluate this new migration metric.
We find that while the precise-M metric decreases flash write I/O by more than 2$\times$ compared to the strawman approach, it almost doubles the CPU utilization, resulting in an overall throughput that is less than 1/3 of the strawman scheme. 
%one third smaller than the strawman scheme.
%This satisfies our goal of lower write amplification. 
%However, this policy almost doubles the CPU utilization.
%This is because computing the precise value of $M$ requires computing the popularity and key overlaps of all the candidate ranges and their SST files.
This is because computing $M$ precisely requires checking the popularity of each object in the tracker, and navigating the indices of all items in the candidate range both in the DRAM B-tree and in the SST file indices, to check for overlaps.
This is CPU-intensive and leads to long migrations (30 seconds). 
%We observe an average migration time of 30 seconds.
% For this experiment where every partition owns around 210 SSTables, we observe an average migration time of 30 seconds.
%Since migration is too slow that it fails to function as an efficient garbage collector, \name has to aggressively rate-limit foreground client writes until its frees enough space on NVM. 
%Figure \ref{fig:mig-design2} shows that while precise-M reduces flash write I/O, its throughput is less than a third of the strawman's. 
% This leads to lower overall throughput of only 49.3 Kops/s, which is less than 1/3 of the strawman approach's. 


% \Paragraph{Optimizations}
\paragrapha{Approximating migration metric.}
%We find that while the new migration metric achieves low flash write I/O, computing the precise value of $M$ is too expensive to meet \name's high-performance goal. 
Therefore, we propose computing a metric called approx-M that efficiently approximates the value of $M$.
Instead of computing the statistics for each individual object in the candidate key range, approx-M metric breaks each partition key space into smaller, fixed-sized ranges, which we call buckets. It then keeps track of approximate values for $p$, $o$, and $F$ in each one of the buckets. %By default, the bucket size in \name, is the same as the key range size (64K keys), so most NVM key ranges will contain 1-2 buckets. 
approx-M can be computed using a weighted average of the parameters of each bucket that overlaps with the candidate key range. 
It therefore provides much better CPU utilization than the precise metric, and better overall throughput than both the strawman scheme and the precise metric. We describe the implementation and maintenance of buckets in \S\ref{sec:mig-metric-impl}.
% We leave the full description of how the buckets are implemented and maintained in \S\ref{sec:mig-metric-impl}.
\subsubsection{Key Range Selection}
% Beyond computing a metric for migration efficiency, a second important design question is which NVM key ranges should be considered as candidates in a migration job. 
A second important design question is which NVM key ranges should be considered as candidates for migration. 
One simple approach is to enumerate over all possible NVM key ranges to decide which to migrate. 
However, this can be impractical for large databases with hundreds of thousand of SST files.
%Therefore, we need a robust key-range selection mechanism that runs in near-constant time and generates a good candidate list. 
Instead, we use power-of-k choices~\cite{power-of-two} to select a subset of migration key ranges as candidates. 
%The more random choices we consider, the better the selected migration key range will be. 
Note that when the database is starting up and there are no SST files on flash, \name will randomly select a range of neighboring unpopular keys, with a total size close to the configured SST file size.
We present an in-depth evaluation of different migration metrics and key-range selection approaches, and discuss their trade-offs in \S\ref{sec:mig-eval}.


% % MJF Doesn't really clarify enough why this is a hard problem. When I read the above, I conclude that:  You migrate the keys that are unpopular according to to clock metric.  But doesn't explain how a naive implementation of this will fair the three above goals.
% %
% % MJF Maybe needs a strawman: How does naive technique fail.  Left comments in Slack about this.  What does "ideal" mean?  In general, I don't like the term "ideal" -> are you sure you don't mind "good enough"?
% Determining what data on NVM to migrate is challenging. 
% Since data on NVM is organized as individual key-value pairs, the search space for an ideal set of migration keys is infinite. 
% In addition, these migration key ranges will always have some overlap with data organized in the granularity of SSTables on QLC. 
% Merging these NVM key-value pairs into existing QLC data inevitably incurs write amplification.
% % MJF Don't like the rhetoric flair
% So, how to achieve efficient migrations?

% We break down the problem into two sub-problems below:
% % MJF First is a phrase, not a sentence. And not a question :)
% \begin{denseenum}
%     \item How to quickly find key ranges to migrate?
%     \item What is an \emph{ideal} migration key range?
% \end{denseenum}

% % MJF I dont' fully undrstand from the text below what a "migration policy" vs. a "migration metric" is?
% \Paragraph{Migration Policy} 
% Migration policy is the mechanism that efficiently walks through the search space and identifies candidate migration key ranges. 
% % MJF bounded / poly time isn't a good metric for high performance systems. A system which takes 100ms or 10 minutes can still be poly time.  What more do we want to say?
% It should finish within bounded time (\ie polynomial time) to meet the time constraint of fast migration. 
% % MJF See comment above -- need to clarify what makes a "good candidate key range"
% A good policy can help reduce the search scope drastically and recognize good candidate key ranges. 


% \Paragraph{Migration Metric} 
% The role of a migration metric is to decide which key range to select out of some candidate migration key ranges. 
% % MJF Could we say "good-ness" rather than "ideal-ness"?  (e.g., "goodness of fit") -> we aren't claiming "ideal" here after all.
% It captures the \emph{ideal-ness} of a migration key range: the higher the value, the better it is for migration.
% The objective of our migration metric is to minimize the QLC write cost per migrated key.
% With this goal, we formulate the migration metric, $M$, as follows:
% \begin{equation}
%     M = \frac{1 - p}{N(1 - s)}
%     \label{eq:migration}
% \end{equation}

% % MJF I would prefer if symbols reflect description:  e.g. t_{n} = total keys in selected NVM,  t_{f} = total keys is selected flash region, u_{n} = unpopular keys in selected NVM, $o$ = overlap, $p$ = popularity, "f" = fanout
% \begin{table}[t!]
%     \centering
%     \small
%     % \begin{tabular}{l{0.2cm}l{1.2cm}l{0.2cm}}
%     \begin{tabular}{p{0.8cm} p{7cm} }
%       \toprule 
%       Symbol & Description\\
%       \midrule
%         $\; X$ & Number of total keys in selected NVM key range. \\
%         %\hline
%         $\; Y$ & Number of total keys in overlapped SSTable on QLC before merging.  \\
%       %\hline
%       $x$ & Number of unpopular keys in selected NVM key range. \\
%       %\hline
%       $s$ & \emph{Overlap ratio}: Fraction of keys [0,1] in SSTable that also appear in selected NVM key range.\\% It is $\in$ [0,1]. \\
%       %\hline
%       $p$ & \emph{Popularity ratio}: Fraction of popular keys [0,1] in selected NVM key range.\\ % It is $\in$ [0,1]. \\
%       %\hline
%       $N$ & \emph{Fanout parameter}: The size ratio $\frac{Y}{X}$ between overlapped SSTable on QLC and selected NVM key range.\\% It equals to \(\frac{Y}{X}\).\\
%       \bottomrule
%     \end{tabular}
%     \caption{Notations}
%     \label{tab:notation}
% \end{table}

% Table~\ref{tab:notation} lists the symbols and their meanings. 
% Section \ref{sec:metric-formula} presents the derivation of Eq \ref{eq:migration}.


% A good metric, together with a fast policy, helps achieve efficient migration by satisfying one or more desired characteristics mentioned above. 
% We present an in-depth evaluation of different migration metrics and policies, and discuss their trade-offs in Section \ref{sec:mig-eval}.


% \todo{change the title to analytical model or something, and condense the part below}

% % MJF awkward that write out "deleted" and "overwritten".  But in general, I rather you derive this less and make sure you explain in english what's going on throughout.
% \subsubsection{Migration Metric Formulation}
% \todo{Skip this, under revision}
% \label{sec:metric-formula}
% Given an NVM key range that overlaps with a SSTable of $Y$ total keys, migrating its $x$ unpopular keys to QLC eventually incurs \((x+Y-deleted-overwritten)\) keys written back to QLC. 
% Thus, the cost to migrate an NVM key is:
% $$
% \frac{x+Y-deleted-overwritten}{x}
% $$

% \noindent We ignore deleted keys in the analysis for simplicity. This cost becomes: 
% \begin{align*} 
% = \frac{x+Y-overwritten}{x} \\
% = Y - \frac{overwritten}{x} 
% \end{align*}

% During migration, older versions of data in the SSTable on QLC will be overwritten when merging with more recent data from NVM.
% If the ratio of overlapped keys in the SSTable is $s$, the number of these overwritten key can be represented as \(Ys\).
% We rewrite the cost as:
% \begin{align*} 
% = \frac{Y - Ys}{x} \\
% = \frac{Y(1-s)}{x} 
% \end{align*}

% The number of unpopular keys migrated, $x$, can be decomposed into simpler terms. 
% Since the NVM key range has $X$ total keys and its percentage of popular keys is $p$, then $x$ is \(X(1-p)\).
% The cost is simplified to:
% \begin{align*} 
% = \frac{Y(1-s)}{X(1-p)} 
% \end{align*}

% Since N is the size fanout parameter, \ie \(\frac{Y}{X}\), we can further reduce the cost formula as:
% \begin{align*} 
% = \frac{N(1-s)}{(1-p)} 
% \end{align*}

% Our goal is to minimize the QLC write cost per NVM key during migration.
% The migration metric, $M$, becomes the inverse of this cost. 
% We will select the NVM key range with highest value of $M$ (\ie the lowest QLC write cost) as the final
% % MJF "champion"?
% champion for migration where
% \begin{align*} 
% M & = \frac{(1-p)}{N(1-s)}
% \end{align*}

% MJF Subsection title should probably be what problem you are solving, not just "upserts".  Something like "Ensuring popularity distributions with Upserts" or something.  Esp. given that the first paragraph
\subsubsection{Object Promotions Under Dynamic Workloads}

During the migration process, objects can be both promoted and demoted. Demotions have an obvious benefit: they free up space in NVM. Promotions, on the other hand, are more expensive, since they take up space in NVM for an object that was previously stored in flash.
However, sometimes objects also need to be promoted from flash to NVM, in order to enable fast reads for popular objects, which at some point got demoted. For example, this would occur when a large burst of newly-written objects fills up NVM. Such bursts have been observed in production workloads~\cite{fb2020,twitter-cache,cliffhanger}. 
%Migration is the main mechanism through which \name does placement of popular objects on NVM. When NVM nears its size threshold, a migration job is triggered. 
%Migrations demote all the unpopular objects in a key range to flash, while retaining the popular objects on NVM. Demotion based migrations have two limitations. Firstly, placement decisions are carried out only for objects that are already on NVM; objects stored on flash stay on flash, even if they are popular. 
%This creates a problem for workloads in which the key popularity for writes and reads comes from different distributions, e.g. uniform writes and zipfian reads as observed in production systems~\cite{fb2020}. Such workloads can fill up NVM quickly and trigger demotions on objects that may not have been read yet. Once those objects move to flash and become popular, they don't get a chance to get placed on NVM, thus leading to poor read performance.

\subsubsection{Read-triggered Migrations}

By default, migrations in \name are triggered when NVM fills up, due to writes.
However, a write-triggered migration is not always suitable for moving items between the two tiers. For example, in read-heavy workloads, NVM will only slowly get filled up, and the write-triggered migration process will not be called frequently enough to keep up with changing read popularity distributions.
Therefore, \name also employs read-triggered migrations for moving items between NVM and flash. The main goal of read-triggered migrations is to improve the ratio of reads served from NVM. 

Read-triggered migration comprises of three stages: detection, invocation, and monitoring. In the detection stage, \name checks if the write-triggered migrations aren't keeping up with popularity distributions. It does so by detecting read-dominated workloads where a large proportion of the keys in the tracker are stored on flash. If so, it triggers read-triggered migrations for an epoch (by default 1~M client operations). At the end of each epoch, the monitoring stage tracks the ratio of reads served from NVM vs. flash. If the migrations that were triggered in the previous epoch improved that ratio above a threshold (by default 1\%), it continues the migrations for next epoch. If not, it enters a cool-down period (by default 10~M operations). At the end of that period, read-triggered migrations resume again from the detection stage. %Promotions in \name can be triggered either by write-triggered or read-triggered migrations.

% \todo{Do we need to add more details for upserts here?  Mike:  Yes. Especially what "if the workload type fits the criteria" -> Where do you define that criteria? What is the ratio?  Goal?  In general, also need to better explain this why.}


%For many read dominated workloads, migrations may not get triggered very often. Without migrations \name cannot execute object placements for popular data resident on flash.



% \subsection{Migration} 
% \label{sec:migration}
% Migration is the background maintenance operation across storage layers in \name. 
% It is triggered to free up space when NVM usage is close to its allocation threshold.
% Similar to compaction in LSMs, migration is a form of garbage collection. 
% In \name, migration plays a central role in achieving the design goals of low read latency and low flash write amplification. Also, in-efficient migrations can stall the foreground client operations and degrade the overall system performance. 
% We detail three desired characteristics of migration in \name below. 

% \Paragraph{Read Popularity Awareness}
% Flash NAND reads can be order of magnitude slower compared to NVM. Migrating popular objects to flash NAND can result in poor read performance. Thus, migration needs to be read popularity aware. Migrations in \name use the mapper to check if an object meets the criteria to be pinned on NVM. Only colder objects are moved to the flash NAND. This ensures that more reads are served from NVM with lower latency.
% %Because reads and writes are of orders of magnitude faster on Optane, \name keeps frequently accessed data on Optane, serving as a secondary cache.
% %Migration should respect such hot-cold data separation.
% %It works together with clock cache to pin popular data on Optane while only migrating colder data to QLC. 
% %This ensures that more reads are served from Optane and delivers lower overall read latency.

% \Paragraph{Low Write Amplification}
% Selection of objects that should be migrated down has a huge impact on the write amplification of the flash NAND. Objects on NVM need to be merge-sorted with their overlapping SST files on flash NAND and then written back as new SST files. A naive selection of objects can result in re-writing all the files in flash NAND.  
% Flash devices are known to have limited write cycles and tend to wear out quickly if write amplification is high. Migrations need to be optimized for low write amplification.

% \Paragraph{Garbage Collection Efficiency}
% The primary goal of migration is to free up space on NVM for new incoming writes.
% Each invocation of migration has a cost, including setup overhead and additional CPU and IO cost. Slow migrations can stall client operations. Migrations need to run fast and be efficient in terms of garbage collection.

% \subsubsection{Migration Metric}
% \label{sec:migration-metric}
% The role of migration metric is to decide which key range to select for migration out of a set of candidate key ranges on optane. 
% The higher the value of migration metric, the more suitable the key range is for migration.
% A good migration metric can help satisfy one or more desired characteristics mentioned above. 
% The objective of our migration metric is to minimize the QLC write cost per migrated key.
% With such a goal, we formulate migration metric, $M$, as follows:

% \begin{equation}
%     M = \frac{1 - p}{N(1 - s)}
%     \label{eq:migration}
% \end{equation}

% \begin{table}[t!]
%     \centering
%     \small
%     % \begin{tabular}{l{0.2cm}l{1.2cm}l{0.2cm}}
%     \begin{tabular}{p{1cm} p{6cm} }
%       \toprule 
%       Symbol & Description\\
%       \midrule
%       $X$ & total number of keys in the selected optane key range \\
%       \hline
%       $Y$ & total number of keys in the overlapped SSTable on qlc before merging  \\
%       \hline
%       $x$ & number of unpopular keys in the selected optane key range \\
%       \hline
%       $s$ & overlap ratio: the percentage of keys in the SSTable that also appear in the selected optane key range. It is $\in$ [0,1]. \\
%       \hline
%       $p$ & popularity ratio: the percentage of popular keys in the selected optane key range. It is $\in$ [0,1]. \\
%       \hline
%       $N$ & fanout parameter: the size ratio between the overlapped SSTable on QLC and the selected optane key range. It equals to \(\frac{Y}{X}\).\\
%       \bottomrule
%     \end{tabular}
%     \caption{Notations}
%     \label{tab:notation}
% \end{table}

% Table~\ref{tab:notation} lists the symbols and their meanings in detail. 
% Below, we show the derivation of Eq \ref{eq:migration}.

% Moving $x$ unpopular keys to qlc eventually incurs \((x+Y-deleted-overwritten)\) keys written to qlc. 
% Thus, the cost to migrate an optane key is:

% $$
% \frac{x+Y-deleted-overwritten}{x}
% $$

% \noindent For now, we ignore deleted keys in the analysis for simplicity. This cost becomes 

% \begin{align*} 
% = \frac{x+Y-overwritten}{x} \\
% = Y - \frac{overwritten}{x} 
% \end{align*}

% During migration, older versions of data on the SSTable on qlc will get overwritten when merging with more recent keys from optane. 
% The number of these overwritten keys can be represented as \((Ys)\).
% We can rewrite the cost as:
% \begin{align*} 
% = \frac{Y - Ys}{x} \\
% = \frac{Y(1-s)}{x} 
% \end{align*}

% We can further decompose $x$ into simpler terms. 
% Given a selected optane key range, $x$ is the number of unpopular keys. 
% Since $p$ is the percentage of popular keys in the optane key range and $X$ is the total number of keys in optane key range, x now becomes \(X(1-p)\).

% The cost further simplifies to:
% \begin{align*} 
% = \frac{Y(1-s)}{X(1-p)} 
% \end{align*}

% Since N is the fanout parameter, that is \(\frac{Y}{X}\), we can further reduce the cost formula as:
% \begin{align*} 
% = \frac{N(1-s)}{(1-p)} 
% \end{align*}

% Therefore, we set our migration metric to be the inverse of this cost:

% \begin{align*} 
% M & = \frac{(1-p)}{N(1-s)}
% \end{align*}

% The goal of our new migration metric is to minimize the QLC write cost per optane key during migration.  
% we will select the optane key range with the highest value of $M$ (aka the lowest qlc write cost) as the final champion for migration. 

 

% \subsubsection{Migration Policy}
% \label{sec:migration-policy}
% Migration policy is the mechanism that tells us how to find a set of candidate key ranges suitable for migrations. 

% \subsection{STOP HERE} 


% In this section, we introduce \name, a read-aware LSM tree. We first discuss design challenges, and then
% detail \name's main design components. In addition, we discuss how to deploy \name in practice.

%Asaf: I'm commenting out this subsection -- all these points should have already been made in sections 2+ 3, we've said this several times already so far.
%\subsection{Assigning LSM Levels to Storage Tiers}
%As discussed, modern storage technologies have two divergent goals: optimizing for performance \vs optimizing for cost. The basic intuition for using different storage technologies  in the same system that vary on the performance-cost spectrum is that, hopefully, these choices would achieve the best of both worlds and navigate the performance-cost curve in a Pareto efficient manner. 

%The basic structure of LSM trees naturally lends itself to storage tiering. Since each level of the tree is subsequently exponentially larger than the previous one~\cite{o1996log,rocksdb-facebook,leveldb}, 
%we can place the LSM tree levels on different storage technologies by descending order of performance (and ascending order of price per bit). %For example, a typical architecture for \name is that the first LSM tier is DRAM, the second tier is a fast storage technology (such as 3D XPoint or Z-NAND), and the remaining tiers are one or more types of flash devices (or even HDDs).
%Since the lower layers have an order of magnitude greater storage capacity that their preceding layers, when \name stores the last layer (or last few layers) using a less expensive technology, its overall cost savings remain significant.

%However, we need to minimize the performance impact of using slower storage at the lower layers. Of particular concern is read performance, as the LSM tree layout is traditionally dictated by write order, not read efficiency. Thus, \name's technical novelty arises from making the LSM tree read-aware, \ie ensuring frequently read objects are more likely to be placed on the higher levels of the tree.

% \name is comprised of three main components (Figure~\ref{fig:prismdb-sys}). The \emph{tracker} is responsible for tracking which objects are popular. The \emph{mapper} keeps track of the distribution of object popularity across the entire LSM tree and translates that distribution to an actionable algorithm for selecting which objects to pin. Then, the \emph{placer} ensures that popular objects remain on higher levels of the LSM tree, where they will be stored on faster storage when using heterogeneous storage.

% Some notes. We need to answer four important design questions.
% Which? Which keys should be pinned?
% Where? Where should those keys be pinned?
% When? When should those keys be pinned?
% How? How should those keys be pinned without violating consistency or impacting throughput?

%Note that as Figure~\ref{fig:clock} shows, it takes the \clock value distribution a few seconds to converge. The distribution initially fluctuates because there are a relatively small number of keys in the tracker, so each eviction cycle of the \clock hand changes the distribution. Thus, by default, \name starts pinning objects only after the tracker is full.

% \subsection{Placer: Pinning Keys to Levels} 
% \label{sec:placer}
% The third component in our system, the \emph{placer}, is responsible for pinning popular keys to LSM levels residing on different storage mediums. 

% Ideally, given our tiered storage design, we would like to keep all hot keys at the top of the LSM tree. However, we need to take into account LSM tree level sizing. Write amplification in LSM trees is minimized when the ratio between the sizes of each subsequent level is fixed across all levels,
% % MJF Can we add something like:
% namely, that level $L_i$ is $k$-times larger than the level $L_{i-1}$, where $k=10$ typically~\cite{o1996log,rocksdbcidr}.
% % ^ I have no idea if this is correct, but would be good.
% This imposes a size constraint on each level, and means that we cannot indiscriminately pin all the hot objects to the top levels that reside on fast storage.
% Deviating from the LSM tree sizing rule can increase the overall write amplification and reduce overall performance, which we also confirmed experimentally.

% %The number of LSM tree levels defines the resolution, or number of popularity groups of the objects in the tracker, and the level sizing rule defines the size of each of those popularity groups.

% Another design goal for the placer is that it must not violate the consistency guarantees of the LSM tree. LSM trees typically maintain consistency by always storing newer versions of objects in upper levels and older versions in the lower levels.  Naively pinning hot keys to top levels---and violating this versioning property---can break the consistency guarantee of LSM trees. (We discuss this further in \S\ref{sec:consistency}.)

% The placer also needs to be lightweight, since it is competing with reads, writes, and background compaction jobs for resources. It should avoid adding any locks on the database since reads and writes are being served concurrently. The timing of when to trigger the pinning process is also important. Ideally, it should be done during periods of reduced database activity to avoid resource contention.

% A popular object that is cached in DRAM may also get pinned by the placer to faster storage (double caching). In this case, pinning is still useful as it enables better hot-cold separation, which in-turn improves dram cache efficiency. Ideally, DRAM cache policy should be optimized to take tiered storage into account. We leave this for future work.

% % Or should we write the above in terms of Design Requirements?
% % R4: Pinning logic that converts the key popularity into a level assignment
% % R5: Pinning logic that doesn’t violate the LSM layer sizing restrictions or consistency
% % R6: Pinning logic that is memory, CPU and disk I/O efficient

% % Talk about the compaction scheme here
% \Paragraph{Pinned Compactions}
% %\label{sec:pinned-compactions}
% To achieve the above stated goals, we combine the pinning logic with the compaction process of LSM. We introduce a new compaction algorithm called \emph{pinned compaction}. Compaction by default moves the keys towards the bottom levels of the tree. Compaction does a merge sort on the SST files between two adjacent levels. In the process, it reads every single key from the SST files and writes them in the sorted order into the output level.
% We extend the new compaction process to not just retaining the popular keys, but also ``pull up'' popular keys stuck in the lower level, possibly on slower storage. We call this process, not found in traditional LSM trees, ``up-compaction.'' %Since compaction is an integral part of the LSM operation, embedding the pinning process in compaction makes pinning a “native” operation. 
% %Doing so obviates the need for allocating separate compute/disk resources for the pinning process and keeps the overall LSM design simple.
% Because each SST file is already sorted, the merge between SST files can be executed in
% an efficient, streaming manner; a property that up-compaction continues to maintain as
% well.

% \begin{figure}
%   \begin{center}
%   {\includegraphics[scale=0.4]{figures/pinned_compaction.pdf}}
%   \end{center}
%   \caption{\label{fig:pinned-compaction} Example of pinned compaction.}
% \end{figure}

% Figure~\ref{fig:pinned-compaction} shows an example of how pinned compactions work on files under compaction. Keys shown in red and gray are present in the tracker; keys in white are not in tracker. Keys 40, 35, and 65 (shown in red) are keys with \clock value 3. Keys in gray have \clock value 2. Assume that the pinning threshold pins all keys with \clock value 3. During the merge process, instead of compacting everything down, key 40 is retained in $L_{i-1}$. Also, popular keys, 35 and 65, from the lower level $L_{i}$ are compacted up and stored in $L_{i}$. 
% At a later time, if the key popularity changes and the keys residing in $L_{i-1}$ either don't satisfy the pinning threshold or are evicted from the tracker, they will be \textit{un-pinned} in the next compaction event and compacted down. Pinned compactions can temporarily generate small SST files comprised of popular keys. At a later point, when \name selects these files again for compaction, they will be merged with other SST files. In our evaluation, we observed that less that 10\% of the SST files in a level were small (less than 10MB).

% \Paragraph{Choosing Which SST File to Compact}
% \label{sec:clock}
% When a compaction job is triggered, it first chooses a level and then an SST file in that level for compaction. With traditional LSM, picking the candidate SST file is based on some system level objective like reclaiming storage space, reducing write amplification, and so forth.

% For \name, we introduce a new SST file selection criteria, which better aligns with 
% the high-level goal of pinning keys to appropriate levels. When the SST file is
% created, a popularity score is assigned to it, based on the \clock values of
% objects present in that file. Objects not present in the tracker get a default
% score of -1. Since by default \clock values range between [0,3], using them
% directly is problematic, since the difference between a highly popular key
% (\clock value 3) and an unpopular key (\clock value -1) is just 4,
% \ie it only take 3 un-popular keys to negate the contribution of a highly popular key.
% % MJF is this a total hack?  Is there something more principles of why you did this?  (i.e., why not ^2 ?  ^4?
% % AR: Kind of a hack :). I tried ^1 and ^2, ^3 worked better..
% We devise a workaround to this problem by using a weight parameter $n$ to boost the contributions of popular keys towards the SST popularity score:
% %\vspace{-0.5ex}
% $$
% score = \Sigma(object_{i}\:clock\:value)^{n}
% $$
% %\vspace{-0.5ex}
% \noindent
% where $i$ is the $i^{th}$ key in the SST file. In our experiments, we use $n=3$.

% During compaction, each SST file in a level is sorted in the ascending order of popularity score, and the file with the lowest score is selected for compaction.
% %Asaf: I am just commenting out the following sentence... Seems unnecessary since we already introduced the algorithm.
% % MJF "pinned" sounds like a binary.  I.e., SST file is "pinned" or not.  Connect is memory pinning.  Here you just mean a "highly-scored" SST file, right?  I'm also then slightly confused by the last sentence.  Why is a "newly written file" --> why can't you handle this by the score of that file?
% % MJF also this sentence is confusing -->  since the _file_ will be retained.  Don't you mean "since most keys belonging to that file will be retained" ?
% %Intuitively, trying to compact a highly scored SST file (\ie one consisting of many popular keys) can result in higher write amplification, since the file will be retained on the same level, and the other compacting files will be read and written unnecessarily.

% \subsection{Maintaining Consistency} 
% \label{sec:consistency}
% LSM-backed databases like RocksDB ensure that database clients will always read the latest version of the object committed to that database. LSMs ensure this behavior by versioning all writes (inserts, updates, or deletes) to a key, where newer versions of the key reside on upper levels of the LSM tree and older versions towards the tree's bottom.  In this regard, when a read query traverses the tree from memtables, to L0, and then on downwards, the first version of the key it encounters is the latest (including a ``tombstone'' record for deletes). Even during compactions, this guarantee is maintained. 

% \name's read-aware LSM tree maintains the same consistency guarantees. If a pinned compaction retains a set of objects in the same level, they will always be the more recent versions of objects than present in the lower levels. Even when objects rise up a level during a pinned compaction, they don't break the LSM guarantee: if the same key is encountered when merging SST files from levels $L_{i-1}$ and $L_i$, 
% the merge process preserves the (newer) key from level $L_{i-1}$.In doing so, read-aware LSM trees continue to ensure the ordering of key versions down the tree.

% \subsection{Deploying \name}

% We envision \name being deployed in two different setups.

% The first setup is on a single physical server, containing more than one type of storage device. Similar to RocksDB, for load balancing purposes, each server would contain multiple instances of \name, each of which would be assigned a certain ratio of each of the storage devices' capacity.
% In this paper, we focus on the NNNTQ setup to demonstrate how it can work with three storage devices. However, \name's design is generalizable to other heterogeneous setups, including a simpler deployment scenario with just two storage tiers, such as NNNNQ. Such a configuration could be readily deployed with two devices (\eg a 280~GB Intel 900P Optane SSD and a 2~TB Intel 760p QLC drive) using a 10:1 level ratio, where about 90\% of the capacity would be allocated to QLC, and the rest to Optane.

% The second setup is a disaggregated storage setting, where there are multiple disaggregated storage tiers, each of which has their own cost and performance characteristics. In this scenario, \name's layers would be split across multiple different disaggregated storage tiers.  Even the major public clouds today all support various forms of such disaggregated storage tiering.

==> design_oldprism.tex <==
%-------------------------------------------------------------------------------
\section{PrismDB Design}
\label{sec:design}
%-------------------------------------------------------------------------------

In this section, we introduce \name, a read-aware LSM tree. We first discuss design challenges, and then
detail \name's main design components. In addition, we discuss how to deploy \name in practice.

%Asaf: I'm commenting out this subsection -- all these points should have already been made in sections 2+ 3, we've said this several times already so far.
%\subsection{Assigning LSM Levels to Storage Tiers}
%As discussed, modern storage technologies have two divergent goals: optimizing for performance \vs optimizing for cost. The basic intuition for using different storage technologies  in the same system that vary on the performance-cost spectrum is that, hopefully, these choices would achieve the best of both worlds and navigate the performance-cost curve in a Pareto efficient manner. 

%The basic structure of LSM trees naturally lends itself to storage tiering. Since each level of the tree is subsequently exponentially larger than the previous one~\cite{o1996log,rocksdb-facebook,leveldb}, 
%we can place the LSM tree levels on different storage technologies by descending order of performance (and ascending order of price per bit). %For example, a typical architecture for \name is that the first LSM tier is DRAM, the second tier is a fast storage technology (such as 3D XPoint or Z-NAND), and the remaining tiers are one or more types of flash devices (or even HDDs).
%Since the lower layers have an order of magnitude greater storage capacity that their preceding layers, when \name stores the last layer (or last few layers) using a less expensive technology, its overall cost savings remain significant.

%However, we need to minimize the performance impact of using slower storage at the lower layers. Of particular concern is read performance, as the LSM tree layout is traditionally dictated by write order, not read efficiency. Thus, \name's technical novelty arises from making the LSM tree read-aware, \ie ensuring frequently read objects are more likely to be placed on the higher levels of the tree.

\name is comprised of three main components (Figure~\ref{fig:prismdb-sys}). The \emph{tracker} is responsible for tracking which objects are popular. The \emph{mapper} keeps track of the distribution of object popularity across the entire LSM tree and translates that distribution to an actionable algorithm for selecting which objects to pin. Then, the \emph{placer} ensures that popular objects remain on higher levels of the LSM tree, where they will be stored on faster storage when using heterogeneous storage.

% Some notes. We need to answer four important design questions.
% Which? Which keys should be pinned?
% Where? Where should those keys be pinned?
% When? When should those keys be pinned?
% How? How should those keys be pinned without violating consistency or impacting throughput?

\begin{figure}
  \begin{center}
  {\includegraphics[scale=0.40]{figures/prismdb_system.pdf}}
  \end{center}
  \caption{\label{fig:prismdb-sys} PrismDB system diagram.}
\end{figure}

\subsection{Tracker: Lightweight Tracking of Keys} 
\label{sec:tracker}
%In the heterogeneous setup, hotter keys should be pinned to faster storage and colder keys should compact down towards the levels residing on slower storage.
The first component in PrismDB, the tracker, is responsible for tracking which objects are frequently read at a low overhead.
There is a large body of work on how to track and estimate object popularity~\cite{LHD,RIPQ,mini-caches,SHARDS,lrb}.
However, many of the existing mechanisms require a relatively large amount of data per object, in order to track various access statistics (number of prior accesses, frequency, relationships with other objects, etc.)~\cite{LHD, lrb}. 
Given that key-value objects are often small (\eg less than 1~KB~\cite{cliffhanger,nishtala2013scaling,fb2020}), we need to limit the amount of metadata we use for tracking purposes per object, yet maintain an accurate prediction on how ``hot'' the object is, or how likely it is to be read or updated in the near future. 
%
In addition, LSM tree implementations support a high number of concurrent write and read operations to the database~\cite{rocksdb-documentation,leveldb}. This requires a high performing popularity tracking mechanism that can track millions of small objects at high throughput.% and to evaluate whether it would provide sufficient information to decide which objects to pin. 

% Or should we write this section in terms of Design Requirements?
% R1: Key tracking mechanism that has sufficient resolution to differentiate between key popularity classes.
% R2: Key tracking mechanism that can track billions of small objects at high throughput.
% R3: Key tracking mechanism that can track billions of small objects at low memory and CPU overhead.

%Caching policies that maintain a full eviction queue (like LRU) are both slow and space inefficient. Eviction queue is implemented as a doubly-linked list with two pointers for each object. Moving recently accessed items to the front of the queue requires global locking. 
\Clock~\cite{clock} is a well-known classical approach that approximates least recently used (LRU) while offering better space efficiency and concurrency~\cite{fan2013memc3,flashield}.
Using a single \clock bit captures recency, while employing multiple \clock
bits can be used to also track frequency. This makes \clock an attractive 
option for estimating the relative popularity of different keys, 
in order to group more popular keys into higher LSM levels.
% The number of LSM levels is an upper bound for the different popularity tiers. 

%Asaf: we should probably add a diagram here, otherwise will be too confusing
\name's tracker implements the multi-bit \clock algorithm for lightweight object tracking across all levels of the LSM.
The tracker uses a concurrent hash map that maps keys to their \clock bits.
%That gives sufficient resolution to capture the heterogeneity of storage in the LSM. 
%In particular, keys get hashed to a bucket. If the bucket has chaining and contains more than one key, then the key is compared to the hash tags. By default, we dedicate 1 byte to the \clock bits and 4 bytes to the hash tag.
% MJF Why 1 byte?  I thought we were only doing 3 \clock levels -> 2 bits? 
% MJF Say why we take the chaining approach vs. something else, like cuckoo hashing?
Each LSM read requires the tracker to update the \clock bits of the object that was read. %Pinning process (described later), uses the key popularity to pin objects to levels and calls Get() on the popular cache. In other systems like Memcached, Get/Set ratio can be imbalanced (30:1) and proposed cache designs~\cite{fan2013memc3} have tried to exploit that imbalance. We don’t observe a noticeable skew in the Get/Set ratio for our cache (TODO: find this ratio for our system). 
Since setting the \clock bits is on the critical path of reads, the set operation needs to be lightweight.  This leads to several performance optimizations in the tracker. 

First, in order to save space, the tracker does not store \clock bits of all key-value pairs in the system, only the most recently read ones.
Second, the tracker is optimized for concurrent key insertions and evictions. 
Traditional \clock implementations use a doubly linked list or a circular buffer that contains the \clock bits along with a hash map that contains the mapping from key to \clock bits, which
% MJF Is "tracker" a 
requires that insertion and eviction operations be serialized. In contrast, \name's tracker does not keep a separate buffer from the hash table. Therefore, it does not require any extra synchronization for those operations, and relies on the synchronization provided by the concurrent hash map. %However, this means we may experience collisions, which will cause the tracker to misidentify a key's \clock bits.
Third, the tracker conducts eviction offline, in a background process, so that when a read causes a new key to be inserted into the tracker and exceed its size, that doesn't trigger eviction of an older key in the critical path. 

% \begin{figure}[!t]
% 	\centering
% % 	\subfloat[]{
% % 	\label{fig:clock-dist}
% % 		\includegraphics[width=0.45\columnwidth]{figures/\clock.pdf}
% % 	}
% 	\subfloat[]{
% 	\label{fig:clock-ycsb}
% 		\includegraphics[width=0.45\columnwidth]{paper/figures/\clock_percents.pdf}
% 	}
% 	\caption{\clock value distributions of \name using the YCSB B workload (Fig.~\ref{fig:clock-dist}). \clock value distribution across all YCSB workloads (Fig.~\ref{fig:clock-ycsb})}
% 	\label{fig:clock}
% \end{figure}

\begin{figure}
    \begin{center}
    {\includegraphics[width=0.55\columnwidth]{figures/clock_percents.pdf}}
    \end{center}
    \caption{Clock value distributions under different workloads.}
    \label{fig:clock}
\end{figure}

% TODO: we are currently using 4byte hash tag per key. Memc3 paper uses just 1byte tag per key. Might be worth checking if 1byte hash improves/worsens performance.

\subsection{Mapper: Enforcing the Pinning Threshold}

Ideally, we could set a ``pinning'' threshold on the popular keys.
That is, at each pass of the compactor, \name should pin some percent (\eg 10\%) of the most popular objects that are being tracked by the tracker to the same level.

However, the actual relative popularity of the object depends on the \clock bit distribution. For example, if \name wants to enforce a pinning threshold of 10\%, and exactly 10\% of keys have all their \clock bits set to 3 (using a two bit \clock, with 3 being most popular and 0 being least popular), then \name should pin all the items with a \clock value of 3. However, if 50\% of the keys have a \clock value of 3, then \name should not pin all items with the \clock value 3, otherwise it will significantly exceed the desired pinning threshold. To illustrate, Figure~\ref{fig:clock} shows that the \clock value distributions change as a function of the workload. 

To this end, the mapper is responsible for keeping track of the \clock value distribution, and uses that distribution to enforce the pinning threshold.
% \todo{Mark: Mapper outputs a global list of to-be-pinned keys that then get pinned to specific levels by the Placer.}
In order to maintain the \clock value distributions, the mapper maintains the aggregate number of keys that have a particular \clock value in an array. 
The array gets updated during insertion and eviction. During eviction, the tracker keeps count of the \clock values of all the items it decremented and the item it evicted and updates the mapper with the new distribution. It also updates the mapper when a new item is inserted into the hash map.

\Paragraph{Pinning Threshold Algorithm}

%With pinned compactions, each key is looked up in the tracker. Depending on the \clock value of the key, the key distribution, and the desired pinning threshold the placer decided whether to pin the key in upper level or to push the key down. 

In order to enforce the pinning threshold, the mapper uses the following algorithm, which is best illustrated with an example. Suppose the \clock distribution is similar to the YCSB-B workload depicted in Figure~\ref{fig:clock},
%(after the distribution stabilizes),
where the percentage of keys with a \clock value of 3 is about 10\%, the percentage of those with a value of 2 is 10\%, the ones with a value of 3 is 30\%, and the remaining 50\% have a \clock value of 0. Suppose the desired pinning threshold is 15\%. If the placer encounters an item with a \clock value of 3, it will always pin it. If it encounters an item with a \clock value
of 2, it will flip a coin whether to keep it or not (in this example, with weight 0.5). If it encounters either an item with \clock value of 1 or 0, or an item that is not currently being tracked (recall the tracker does not track all items in the database), that item will be compacted down.

To summarize, the mapper satisfies the pinning threshold using the highest-ranked \clock items by descending rank, and if need be, randomly samples objects that belong to the lowest \clock value that is needed to satisfy the threshold.  

% MJF Not the right figure
%Note that as Figure~\ref{fig:clock} shows, it takes the \clock value distribution a few seconds to converge. The distribution initially fluctuates because there are a relatively small number of keys in the tracker, so each eviction cycle of the \clock hand changes the distribution. Thus, by default, \name starts pinning objects only after the tracker is full.

\subsection{Placer: Pinning Keys to Levels} 
\label{sec:placer}
The third component in our system, the \emph{placer}, is responsible for pinning popular keys to LSM levels residing on different storage mediums. 

Ideally, given our tiered storage design, we would like to keep all hot keys at the top of the LSM tree. However, we need to take into account LSM tree level sizing. Write amplification in LSM trees is minimized when the ratio between the sizes of each subsequent level is fixed across all levels,
% MJF Can we add something like:
namely, that level $L_i$ is $k$-times larger than the level $L_{i-1}$, where $k=10$ typically~\cite{o1996log,rocksdbcidr}.
% ^ I have no idea if this is correct, but would be good.
This imposes a size constraint on each level, and means that we cannot indiscriminately pin all the hot objects to the top levels that reside on fast storage.
Deviating from the LSM tree sizing rule can increase the overall write amplification and reduce overall performance, which we also confirmed experimentally.

%The number of LSM tree levels defines the resolution, or number of popularity groups of the objects in the tracker, and the level sizing rule defines the size of each of those popularity groups.

Another design goal for the placer is that it must not violate the consistency guarantees of the LSM tree. LSM trees typically maintain consistency by always storing newer versions of objects in upper levels and older versions in the lower levels.  Naively pinning hot keys to top levels---and violating this versioning property---can break the consistency guarantee of LSM trees. (We discuss this further in \S\ref{sec:consistency}.)

The placer also needs to be lightweight, since it is competing with reads, writes, and background compaction jobs for resources. It should avoid adding any locks on the database since reads and writes are being served concurrently. The timing of when to trigger the pinning process is also important. Ideally, it should be done during periods of reduced database activity to avoid resource contention.

A popular object that is cached in DRAM may also get pinned by the placer to faster storage (double caching). In this case, pinning is still useful as it enables better hot-cold separation, which in-turn improves dram cache efficiency. Ideally, DRAM cache policy should be optimized to take tiered storage into account. We leave this for future work.

% Or should we write the above in terms of Design Requirements?
% R4: Pinning logic that converts the key popularity into a level assignment
% R5: Pinning logic that doesn’t violate the LSM layer sizing restrictions or consistency
% R6: Pinning logic that is memory, CPU and disk I/O efficient

% Talk about the compaction scheme here
\Paragraph{Pinned Compactions}
%\label{sec:pinned-compactions}
To achieve the above stated goals, we combine the pinning logic with the compaction process of LSM. We introduce a new compaction algorithm called \emph{pinned compaction}. Compaction by default moves the keys towards the bottom levels of the tree. Compaction does a merge sort on the SST files between two adjacent levels. In the process, it reads every single key from the SST files and writes them in the sorted order into the output level.
We extend the new compaction process to not just retaining the popular keys, but also ``pull up'' popular keys stuck in the lower level, possibly on slower storage. We call this process, not found in traditional LSM trees, ``up-compaction.'' %Since compaction is an integral part of the LSM operation, embedding the pinning process in compaction makes pinning a “native” operation. 
%Doing so obviates the need for allocating separate compute/disk resources for the pinning process and keeps the overall LSM design simple.
Because each SST file is already sorted, the merge between SST files can be executed in
an efficient, streaming manner; a property that up-compaction continues to maintain as
well.

\begin{figure}
  \begin{center}
  {\includegraphics[scale=0.4]{figures/pinned_compaction.pdf}}
  \end{center}
  \caption{\label{fig:pinned-compaction} Example of pinned compaction.}
\end{figure}

Figure~\ref{fig:pinned-compaction} shows an example of how pinned compactions work on files under compaction. Keys shown in red and gray are present in the tracker; keys in white are not in tracker. Keys 40, 35, and 65 (shown in red) are keys with \clock value 3. Keys in gray have \clock value 2. Assume that the pinning threshold pins all keys with \clock value 3. During the merge process, instead of compacting everything down, key 40 is retained in $L_{i-1}$. Also, popular keys, 35 and 65, from the lower level $L_{i}$ are compacted up and stored in $L_{i}$. 
At a later time, if the key popularity changes and the keys residing in $L_{i-1}$ either don't satisfy the pinning threshold or are evicted from the tracker, they will be \textit{un-pinned} in the next compaction event and compacted down. Pinned compactions can temporarily generate small SST files comprised of popular keys. At a later point, when \name selects these files again for compaction, they will be merged with other SST files. In our evaluation, we observed that less that 10\% of the SST files in a level were small (less than 10MB).

\Paragraph{Choosing Which SST File to Compact}
\label{sec:clock}
When a compaction job is triggered, it first chooses a level and then an SST file in that level for compaction. With traditional LSM, picking the candidate SST file is based on some system level objective like reclaiming storage space, reducing write amplification, and so forth.

For \name, we introduce a new SST file selection criteria, which better aligns with 
the high-level goal of pinning keys to appropriate levels. When the SST file is
created, a popularity score is assigned to it, based on the \clock values of
objects present in that file. Objects not present in the tracker get a default
score of -1. Since by default \clock values range between [0,3], using them
directly is problematic, since the difference between a highly popular key
(\clock value 3) and an unpopular key (\clock value -1) is just 4,
\ie it only take 3 un-popular keys to negate the contribution of a highly popular key.
% MJF is this a total hack?  Is there something more principles of why you did this?  (i.e., why not ^2 ?  ^4?
% AR: Kind of a hack :). I tried ^1 and ^2, ^3 worked better..
We devise a workaround to this problem by using a weight parameter $n$ to boost the contributions of popular keys towards the SST popularity score:
%\vspace{-0.5ex}
$$
score = \Sigma(object_{i}\:clock\:value)^{n}
$$
%\vspace{-0.5ex}
\noindent
where $i$ is the $i^{th}$ key in the SST file. In our experiments, we use $n=3$.

During compaction, each SST file in a level is sorted in the ascending order of popularity score, and the file with the lowest score is selected for compaction.
%Asaf: I am just commenting out the following sentence... Seems unnecessary since we already introduced the algorithm.
% MJF "pinned" sounds like a binary.  I.e., SST file is "pinned" or not.  Connect is memory pinning.  Here you just mean a "highly-scored" SST file, right?  I'm also then slightly confused by the last sentence.  Why is a "newly written file" --> why can't you handle this by the score of that file?
% MJF also this sentence is confusing -->  since the _file_ will be retained.  Don't you mean "since most keys belonging to that file will be retained" ?
%Intuitively, trying to compact a highly scored SST file (\ie one consisting of many popular keys) can result in higher write amplification, since the file will be retained on the same level, and the other compacting files will be read and written unnecessarily.

\subsection{Maintaining Consistency} 
\label{sec:consistency}
LSM-backed databases like RocksDB ensure that database clients will always read the latest version of the object committed to that database. LSMs ensure this behavior by versioning all writes (inserts, updates, or deletes) to a key, where newer versions of the key reside on upper levels of the LSM tree and older versions towards the tree's bottom.  In this regard, when a read query traverses the tree from memtables, to L0, and then on downwards, the first version of the key it encounters is the latest (including a ``tombstone'' record for deletes). Even during compactions, this guarantee is maintained. 

\name's read-aware LSM tree maintains the same consistency guarantees. If a pinned compaction retains a set of objects in the same level, they will always be the more recent versions of objects than present in the lower levels. Even when objects rise up a level during a pinned compaction, they don't break the LSM guarantee: if the same key is encountered when merging SST files from levels $L_{i-1}$ and $L_i$, 
the merge process preserves the (newer) key from level $L_{i-1}$.In doing so, read-aware LSM trees continue to ensure the ordering of key versions down the tree.

\subsection{Deploying \name}

We envision \name being deployed in two different setups.

The first setup is on a single physical server, containing more than one type of storage device. Similar to RocksDB, for load balancing purposes, each server would contain multiple instances of \name, each of which would be assigned a certain ratio of each of the storage devices' capacity.
In this paper, we focus on the NNNTQ setup to demonstrate how it can work with three storage devices. However, \name's design is generalizable to other heterogeneous setups, including a simpler deployment scenario with just two storage tiers, such as NNNNQ. Such a configuration could be readily deployed with two devices (\eg a 280~GB Intel 900P Optane SSD and a 2~TB Intel 760p QLC drive) using a 10:1 level ratio, where about 90\% of the capacity would be allocated to QLC, and the rest to Optane.

The second setup is a disaggregated storage setting, where there are multiple disaggregated storage tiers, each of which has their own cost and performance characteristics. In this scenario, \name's layers would be split across multiple different disaggregated storage tiers.  Even the major public clouds today all support various forms of such disaggregated storage tiering.

==> impl_oldprism.tex <==
%-------------------------------------------------------------------------------
\section{Implementation}
\label{sec:impl}
%-------------------------------------------------------------------------------

We implemented 
%\name\footnote{https://github.com/ashwiniraina/ra-lsm} 
\name\footnote{GitHub link elided for anonymity purposes.}
on top of RocksDB v6.2.0, which is written in C++. 
% TODO XXX Add number of lines of code XXX. 
% We also integrated the modified RocksDB  into MyRocks v5.6~\cite{myrocks-blog} for Linkbench~\cite{linkbench} experiments. 
The tracker is built on the concurrent hash map implementation from Intel's TBB library~\cite{tbb}.

\begin{figure}
      \begin{center}
      {\includegraphics[scale=0.25]{figures/clock_operation.pdf}}
      \end{center}
      \caption{\label{fig:clock-operation} PrismDB component interaction}
\end{figure}

% \textbf{KeyCache Implementation}

Intel's TBB concurrent hash map implements a hash table with chaining. Chained hashing offers constant-time insert operations; however, lookup and delete operations may be slower. In our system, inserts to the hash table happen on the read critical path, while lookups and deletes happen in the background. Additionally, the ratio of inserts to lookups in the tracker is 18:1, which makes hash chaining a good fit. In microbenchmarks, we found it took less than 2$\mu s$ to insert a new key into the tracker.

The hash map index is the object key and each index stores a 1~byte value. The top two bits are used for storing the \clock value, while the bottom six bits store the last six bits of the hash of the key version. Multiple versions of the same client key can exist in the LSM, but only the latest version is useful for pinning objects. %The tracker ideally should cache the most recent key version. LSM versions can be up to 8 bytes in size. Storing six bits of the hash value of the version provides sufficient resolution to distinguish between versions.

% \begin{algorithm}
%     \caption{Pseudo code for SET}\label{euclid}
%     \begin{algorithmic}
%     \Procedure{SET(key, version)}{}
%     % \Begin
%     \State $\textit{clock_value} \gets \text{1}$
%     \If {$KEY not in \textit{Tracker}$} \Return false
%     \EndIf
%     \State $j \gets \textit{patlen}$
%     \State $i \gets i+\max(\textit{delta}_1(\textit{string}(i)),\textit{delta}_2(j))$.
%     % \End
%     \EndProcedure
%     \end{algorithmic}
% \end{algorithm}

Figure~\ref{fig:clock-operation} shows the interaction between \name's different design components. When a database client calls the \texttt{get} API, the key is inserted into the tracker. Typically an insert operation also invokes an eviction. However, since the tracker \texttt{insert} is on the critical path of reads for \name, we defer the evictions to a background thread. If the key is not present in tracker, \texttt{insert} writes the key with an initial \clock value of 1. Setting the initial value to 3 can result in keys that are accessed only once staying in the tracker for a long time, since the \clock value needs to get decremented down to 0 before the key is evicted. For a key that is already present in tracker, if its version matches the tracker's version, then the \clock value is set to 3; otherwise, it is treated as a new key.% and the \clock value is initialized to 1. %Keys can experience different \clock value transitions, e.g. \clock transition for one-hit keys (accessed only once), is <1, 0, eviction>, for a very popular key <1, 3, 3, 3..> and for a popular that turns cold later on <1, 3, 2, 1, 0, eviction>.

A background eviction thread implements the \clock hand movement using an iterator over the hash table. Note that new inserts into tracker can happen concurrently while the background iterator is running, by relying on TBB’s concurrent hash map guarantee~\cite{tbb-map} that as long as erase operations are serialized, an iterator running in one thread does not conflict with insert operations happening in other threads. The limitation of running concurrently is that the iterator may either miss visiting some items or visit them more than once within a full iteration. This makes our implementation an approximation of the \clock algorithm. In the context of our system, such approximate behavior does not affect system performance. Finally, the \clock value is stored as an atomic variable. Thus \texttt{lookup} does not need to be serialized with eviction.

Each client \texttt{get} updates the \clock value distribution in the mapper. The mapper is implemented as an array of four atomic integers; each keeps track of the number of keys with a particular \clock value.%, \eg index 0 counts the number of keys in tracker currently with \clock value 0. 
%This generates a real-time distribution of \clock values in tracker. 
While running pinned compactions, the placer calls \texttt{lookup} to check if the key is present in tracker. If so, it queries the mapper to determine whether to pin the key to the current level.


% \begin{algorithm}
%   \caption{Pseudo code for Tracker SET and eviction}\label{euclid}
% % \SetKwInput{KwInput}{Input}
% % \SetKwInput{KwOutput}{Output}
%   \DontPrintSemicolon
% %   \KwInput{Your Input}
% %   \KwOutput{Your output}
% %   \KwData{Testing set $x$}

% % Set Function Names
%   \SetKwFunction{FSet}{ SET}
%   \SetKwFunction{FTracker}{ TRACKER\_THREAD}
 
% % Write Function with word ``Function''
%   \SetKwProg{Fn}{}{:}{}
%   \Fn{\FSet{$key$, $version$}}{
%         clock = 1\;
%         t\_version, t\_clock = \textbf{tracker\_lookup}(\textit{key})\;
        
%         if \textit{key} not found\;
%           \hspace{0.4cm} clock = 1\;
%           \hspace{0.4cm} t\_value = (clock $\ll$ 6) \&\& \textit{version}\;
%           \hspace{0.4cm} \textbf{tracker\_insert}(\textit{key}, t\_value)\;
%         else\;
%           \hspace{0.4cm} if (\textit{version} \&\& 0x3F) == t\_version\;
%             \hspace{0.4cm}\hspace{0.4cm} clock = max(t\_clock+1, 3)\;
%           \hspace{0.4cm} t\_value = (clock $\ll$ 6) \&\& \textit{version}\;
%           \hspace{0.4cm} \textbf{tracker\_update}(\textit{key}, t\_value)\;\;
        
%         if \textit{tracker} capacity exceeds threshold\;
%         \hspace{0.4cm} \textbf{notify\_tracker\_thread}()\;
%         \KwRet\;
%   }
%   \;
  
%   % Write Function with word ``Function''
%   \SetKwProg{Fn}{}{:}{}
%   \Fn{\FTracker{}}{
%         while (true)\;
%           \hspace{0.4cm} for key, t\_value in \textit{tracker}\;
%           \hspace{0.4cm}\hspace{0.4cm} if \textit{tracker} capacity below threshold\;
%             \hspace{0.4cm}\hspace{0.4cm}\hspace{0.4cm} wait()\;
%           \hspace{0.4cm}\hspace{0.4cm}else\;
%             \hspace{0.4cm}\hspace{0.4cm}\hspace{0.4cm} if t\_value != 0\;
%               \hspace{0.4cm}\hspace{0.4cm}\hspace{0.4}\hspace{0.4cm}\hspace{0.4cm} \textbf{tracker\_decrement\_clock}(key)\;
%             \hspace{0.4cm}\hspace{0.4cm}\hspace{0.4cm}else\;
%               \hspace{0.4cm}\hspace{0.4cm}\hspace{0.4cm}\hspace{0.4cm} \textbf{tracker\_evict}(key)\;
%         \KwRet\;
%   }
%   \label{tracker-code}
% \end{algorithm}



==> lsm-perf_oldprism.tex <==
%-------------------------------------------------------------------------------
\section{LSM Performance on Emerging Storage}
\label{sec:perf}
%-------------------------------------------------------------------------------


% Data for block cache enabled
    %   NNNNN & 289 & 10291 & 9 & 121 \\
    %   NNNNT & 109 & 866 & 67 & 125 \\
    %   NNNNQ & 49 & 463 & 133 & 135 \\
    %   NNNTT & 91 & 98 & 67 & 151 \\
    %   NNNTQ & 37 & 36 & 134 & 160 \\
    %   NNNQQ & 25 & 98 & 134 & 224 \\
    %   NNTTT & 89 & 36 & 68 & 194 \\
    %   NNTTQ & 40 & 36 & 134 & 204 \\
    %   NNQQQ & 23 & 36 & 135 & 378 \\
    %   NTTTT & 89 & 36 & 69 & 208 \\
    %   NTTTQ & 36 & 36 & 135 & 218 \\
    %   NQQQQ & 23 & 36 & 137 & 426 \\
    %   TTTTT & 89 & 309 & 69 & 217 \\
    %   QQQQQ & 22 & 103 & 139 & 456 \\

% Data for block cache disabled
    %   NNNNN & 289 & 10291 & 27 & 121 \\
    %   NNNNT & 109 & 866 & 85 & 125 \\
    %   NNNNQ & 49 & 463 & 151 & 135 \\
    %   NNNTT & 91 & 98 & 125 & 151 \\
    %   NNNTQ & 37 & 36 & 192 & 160 \\
    %   NNNQQ & 25 & 98 & 239 & 224 \\
    %   NNTTT & 89 & 36 & 164 & 194 \\
    %   NNTTQ & 40 & 36 & 231 & 204 \\
    %   NNQQQ & 23 & 36 & 322 & 378 \\
    %   NTTTT & 89 & 36 & 189 & 208 \\
    %   NTTTQ & 36 & 36 & 256 & 218 \\
    %   NQQQQ & 23 & 36 & 377 & 426 \\
    %   TTTTT & 89 & 309 & 203 & 217 \\
    %   QQQQQ & 22 & 103 & 406 & 456 \\
    

%LSM performance on heterogeneous flash storage isn’t well studied. Past works~\cite{novelsm} have proposed using non-volatile memories~\cite{optane,znand} for storing some components of the LSM, like Write-Ahead LOG (WAL). Others ~\cite{mutant} have proposed a data tiering model for LSM based on the read popularity of SST files. Prior work fails to capture the LSM level dynamics and caching behavior of LSM trees.

This section presents an evaluation of LSM tree performance on both homogeneous and heterogeneous
storage, and highlight the shortcomings 
of existing LSM tree design when attempting to utilize heterogeneous storage. Throughout the paper,
we use RocksDB, an open-source key-value store built by Facebook~\cite{fb2020}, as our baseline LSM tree implementation.


\subsection{Homogeneous Storage}

We first evaluate RocksDB on a homogeneous, single-disk setup using the YCSB benchmark. We compare its performance on three homogeneous configurations: Optane, TLC, and QLC. Figure~\ref{fig:hom-vs-het} shows the throughput and read latency of running RocksDB on these varying technologies. RocksDB running on Optane has roughly 3.5$\times$ and 5.9$\times$ higher throughput compared to TLC and QLC, respectively. 
 %TODO: say something about read latencies Figure~\ref{fig:hom-vs-het-read-latency} and Figure~\ref{fig:hom-vs-het-update-latency}

% \begin{figure}
%     \begin{center}
%     {\includegraphics[scale=0.3]{figures/hom_vs_het_tput.pdf}}
%     \end{center}
%     \caption{RocksDB throughput on homogeneous and heterogeneous storage under YCSB zipfian 0.99 distribution with 95:5 read-update ratio.}
%     \label{fig:hom-vs-het}
% \end{figure}

\begin{figure}[!t]
	\centering
	\subfloat[]{
	\label{fig:hom-vs-het}
		\includegraphics[width=0.45\columnwidth]{figures/hom_vs_het_tput.pdf}
	}
	\subfloat[]{
	\label{fig:lsm-het}
		\includegraphics[width=0.45\columnwidth]{figures/lsm_het.pdf}
	}
	\caption{RocksDB throughput utilizing homogeneous and heterogeneous storage (Fig.~\ref{fig:hom-vs-het}). Throughput is measured under YCSB-B workload: 95\% read-5\% update, 200 million key dataset, 24 clients, 2 billion requests.  Heterogenous storage configuration (Fig~\ref{fig:lsm-het}) uses Optane for L0-L2 (2.4GB), TLC for L3 (20GB), and QLC for L4 (200GB).}
	\label{fig:io-stats}
\end{figure}

% \begin{figure}
%   \begin{center}
%   {\includegraphics[scale=0.3]{figures/hom_vs_het_read_latency.png}}
%   \end{center}
%   \caption{\label{fig:hom-vs-het-read-latency} Read latency on homogeneous vs heterogeneous storage}
% \end{figure}

% \begin{figure}
%   \begin{center}
%   {\includegraphics[scale=0.3]{figures/hom_vs_het_update_latency.png}}
%   \end{center}
%   \caption{\label{fig:hom-vs-het-update-latency} Update latency homogeneous vs heterogeneous storage}
% \end{figure}

\begin{figure}[!t]
	\centering
	\subfloat[]{
	\label{fig:ycsb-writes}
	\includegraphics[width=0.45\columnwidth]{figures/comp_wr_stats_level_norm.pdf}
	}
	\subfloat[]{
	\label{fig:ycsb-reads}
		\includegraphics[width=0.45\columnwidth]{figures/lsm_read_location.pdf}
	}
	\caption{Distribution of writes and reads across LSM levels (L0-L4), memtable (mt) and block cache (bc) under YCSB-B workload: 95\% read-5\% update, 200 million key dataset, 24 clients, 2 billion requests.}
	\label{fig:io-stats}
\end{figure}

% Below paragraph goes with Linkbench results, not YCSB (duplicate lines)
%As observed in Figure~\ref{fig:ycsb-writes}, access patterns to different LSM tree levels are not homogeneous: on the one hand, the storage cells on the upper levels get read from and written to much more frequently than the lower levels. On the other hand, the lower levels store orders of magnitude more data, and that data is much more static (\ie it is not updated frequently). 

We make the observation that while an LSM tree is a single logical data structure, each one of its levels has very different performance and endurance requirements, as depicted in Figure~\ref{fig:io-stats}. Objects stored in the upper levels of the LSM are read and updated more often than objects stored at the bottom layers. Therefore, the higher levels would benefit from using a high performance and high endurance (and more expensive) storage medium such as NVM. The lower levels on the other hand, which store 90\% or more of the data, can use a much cheaper form of storage such as QLC NAND. In addition, since they are updated much less frequently, they may meet the endurance requirements of cheaper flash storage.  On the other hand, QLC has much slower read latency, so query latency can suffer if a high fraction of reads are served from L4 (as in Figure~\ref{fig:ycsb-reads}).

\begin{figure}
  \begin{center}
  \includegraphics[width=0.85\columnwidth]{figures/cost_vs_read_lat_sim_bigdots.pdf}
  \end{center}
  \vspace{-1ex}
  \caption{ Simulation of trade-off between average read latency and storage cost when storing data in an LSM tree, with a minimum storage lifetime constraint of 3 years. The percentage of reads and writes to each level is based on RocksDB production data~\cite{rocksdbcidr} with a total database size of 223~GB. The hardware configuration is represented by a five-tuple, corresponding to each level of the LSM tree, where
$N$ is Optane SSD (NVM), $T$ is TLC, and $Q$ is QLC. %For example, NNNTQ corresponds to L0-L2 of Optane, L3 of TLC, and L4 of QLC. 
Blue represents homogeneous configurations, and the red configuration is used as the default one in this paper.}
\label{fig:simulation}
\end{figure}

% \begin{figure*}[!t]
% 	\centering
% 	\subfloat[][\textbf{Without DRAM Caching}]{
% 	\label{fig:simulation-nobc}
% 		\includegraphics[width=0.8\columnwidth]{figures/cost_read_lat_sim.pdf}
% 	}\hspace{1cm}
% 	\subfloat[][\textbf{With DRAM Caching}]{
% 	\label{fig:simulation-bc}
% 		\includegraphics[width=0.8\columnwidth]{figures/cost_vs_read_lat_sim_bc.pdf}
% 	\label{fig:simulation}
% 	}

% \caption{Simulation of the trade-off between average read latency (in $\mu$s) and storage cost (cents per GB) when storing data in an LSM tree, with a minimum storage lifetime constraint of 3 years. Percentages of reads and writes across LSM levels are based on RocksDB production data~\cite{rocksdbcidr} for a total database size of 223~GB. The result of each possible hardware configuration is shown in the figure.  The hardware configuration is represented by a five-tuple, corresponding to each level of the LSM tree, where
% $N$ is Optane SSD (NVM), $T$ is TLC SSD, and $Q$ is QLC SSD. %For example, NNNTQ corresponds to L0-L2 of Optane, L3 of TLC, and L4 of QLC. 
% Blue represents homogeneous configurations, and the red configuration ($NNNTQ$) is used as the default one in this paper.} 
% \label{fig:simulation}
% \end{figure*}

\subsection{Heterogeneous Storage}
\label{sec:hetro-perf}

% \begin{figure}
%   \begin{center}
%   {\includegraphics[scale=0.3]{figures/lsm_het.pdf}}
%   \end{center}
%   \caption{\label{fig:lsm-het} LSM on a heterogeneous storage setup}
% \end{figure}

We next examine how well the LSM tree performs on a heterogeneous setup. The LSM tree running on heterogeneous storage is referred to as \emph{LSM-het} for the remainder of the paper. We use a 5-level LSM tree, where each level can be mapped to a different storage tier.
In Figure~\ref{fig:simulation}, we simulate the cost vs. performance trade off of different configurations, by simulating the read latency and cost of each level, when they are placed on different storage technologies. Note that the read latency is computed by taking the average read latency of each storage device measured by Fio, and does not consider tail latencies or any database software overhead (\eg due to lock contention or bloom filter false positives). The simulator is intended to provide a qualitative comparison of the trade off between different heterogeneous configurations.

In order to simulate endurance constraints, we assume the storage devices need to last for at least 3 years, which is a typical lifetime for storage devices. Therefore, if a particular storage technology has been written to too much to last 3 years, we add additional spare storage capacity to that technology until we reach enough storage to achieve the 3 year limit. This method follows the same principle used by enterprise flash devices, which are provisioned with spare capacity to achieve higher endurance for write-heavy workloads.

The ideal points on the Pareto frontier of the curve, as expected, are those where upper levels use the same or a faster storage technology than the lower levels.
In the paper, we examine one of the points on the Pareto frontier, $NNNTQ$,  (depicted in
Figure~\ref{fig:lsm-het}), which maps LSM levels L0-L2 to NVM, L3 to TLC, and L4 to QLC, which contains the key space of the entire database.  %As we can see in our simulations from Figure~\ref{fig:simulation}, $NNNTQ$ provides a good cost-performance tradeoff (falling on the Pareto curve).

We modified RocksDB to map different levels onto different storage types, and again evaluate its performance with the YCSB~\cite{ycsb} benchmark. We observed that even though LSM-het has faster storage components, it performs only marginally better than an LSM that is fully mapped to the slowest storage QLC (Figure~\ref{fig:hom-vs-het}), and it has about 5.8$\times$ worse throughput compared to the LSM running fully on Optane. In short: a heterogeneous RocksDB configuration pays the extra cost of faster storage but does not achieve any significant performance boost.

\begin{figure}[!t]
	\centering
	\subfloat[]{
	\label{fig:rocksdb-heatmap}
		\includegraphics[width=0.48\columnwidth]{figures/rocksdb_heat_map_100k.pdf}
	}
	\subfloat[]{
	\label{fig:prismdb-heatmap}
		\includegraphics[width=0.48\columnwidth]{figures/prismdb_heat_map_100k.pdf}
	}
% 	\newline
% 	\subfloat[]{
% 	\label{fig:prismdb-heatmap-disagg}
% 		\includegraphics[width=0.45\columnwidth]{figures/rocksdb_heat_map_100k_disagg.pdf}
% 	}
% 	\subfloat[]{
% 	\label{fig:prismdb-heatmap-disagg}
% 		\includegraphics[width=0.45\columnwidth]{figures/prismdb_heat_map_100k_disagg.pdf}
% 	}
	\caption{Heat map showing the percentage of reads served by different levels of the 100,000 most popular keys for RocksDB (Fig.~\ref{fig:rocksdb-heatmap}) and \name (Fig.~\ref{fig:prismdb-heatmap}).}
	\label{fig:heatmap}
\end{figure}

% \begin{table}
%     \centering
%   %  \footnotesize
%     \setlength{\tabcolsep}{0.38em}
%     %\begin{tabular}{p{1.5cm}p{1.1cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}}
%      \begin{tabular}{l r r r r r r}
%       \toprule 
%       Benchmark & Memtable & L0 & L1 & L2 & L3 & L4\\
%       \midrule
%       YCSB & 25\% & 3\% & 2\% & 5\% & 16\% & 49\% \\
%     %   LinkBench & 7\% & 4\% & 4\% & 14\% & 19\% & 52\% \\
%       \bottomrule
%     \end{tabular}
%     \caption{Distribution of point read queries across LSM levels with block cache disabled. Block cache is only effective at caching objects present in upper levels (Figure~\ref{fig:ycsb-reads}).}
%     \label{tab:read-dist}
%   \end{table}


% Figure~\ref{fig:heat-map} provides some insights into why heterogeneous LSM doesn’t benefit from faster storage. We track the final read location of top-10000 read-popular keys and plot it as a heatmap.- (No space for heat map)

Why the lack of performance improvement?
Figure~\ref{fig:rocksdb-heatmap} shows a significant number of read queries for top-100K popular keys are served from either L3 and L4 levels, which are mapped on slower storage. This completely diminishes the impact that the faster storage tier would have on read latency. Optimizing LSM trees for heterogeneous storage can be thought of a multi-tiered storage problem, where the first tier is DRAM, the second  is NVM, and the remaining are one or more types of flash devices (or even HDDs). 
Yet we cannot rely on LSM’s traditional design to organize the tree into an efficient multi-tiered storage system, since it does not try to keep popular objects in higher levels of the LSM tree. In \S\ref{sec:design}, we show how we can transform the existing LSM data structure to account for the read performance of different storage technologies using our new \emph{pinned compaction} technique. Figure~\ref{fig:prismdb-heatmap} shows how pinned compactions are effective at keeping popular keys in upper LSM levels,  and serve more read queries from faster storage.

\subsection{Caching Efficiency}
\label{sec:cache-eff}

Single and multi-disk experiments show that it is critical to consider LSM level dynamics while deploying LSM trees over heterogeneous storage. We now turn to another crucial aspect: the caching dynamics of LSM tree systems. 

As discussed in \S\ref{sec:object-placement}, LSM trees cache at a block granularity (4~KB or more) to maximize I/O utilization. However, typical key-value pairs in production workloads are on the order of tens to hundreds of bytes~\cite{fb2020,nishtala2013scaling,rocksdbcidr}. Since the layout of keys within blocks is only dependent on writes, \emph{SST blocks contain objects with different read popularity}. Figure ~\ref{fig:rocksdb-heatmap} shows that the popular keys are scattered across different levels of the LSM and SST blocks.

%Past work~\cite{triad} has proposed separating hold and cold objects in memory before flushing to disk as separate SST files. However, once the files get merged during compaction among different storage levels, they will lose the hot-cold separation. 
Therefore, LSM tree block-level caching turns out to be less effective, as a significant percentage of the objects in the
block cache may not be popular. 
%To improve Blockcache efficiency, key movement decisions within the LSM tree need to be cognizant of reads. None of the existing LSM designs support organizing the keys within the LSM tree based on both writes as well as reads. 
This general limitation of LSM trees affects both the homogeneous
and heterogeneous storage setups and is a key aspect of our design.
%, but its impact is more acute in the heterogeneous case.
% Asaf: why is the blockcache limitation more accute in the hetrogeneous storage setup? Not sure I agree?
%Since most persistent storage is block based i.e. the application can only read at a block granularity. Modern SSDs tend to offer higher throughputs for bigger sized read operations. Block sizes can range from 4KB to 32KB. Production systems typically run with larger block sizes~\cite{rocksdb-comp}. However, it is very common to have key-value sizes in the order of tens or hundreds of bytes~\cite{fb2020}. This mismatch in block size and individual key value size can result in inefficient utilization of DRAM for block cache.

% This paragraph is bit fuzzy, plot is not correct

% Consider a database with 100~M keys, an average key-value pair size of 128~B and SST block size of 8~KB. One SST block can hold up to 64 keys, but not all keys may be frequently read. If a client issues a read for one of the keys in that block, the entire block is fetched into block cache. Figure~\ref{fig:xxx} shows how the density of popular keys within a block affects the block cache efficiency. The ``factor’’ parameter refers to how many versions of the same key are present in the database. It is a proxy for how big the database is compared to the key range of the shard. For example, the 100M data base with key-value pair size of 128~B in the best case should only occupy 12.8~GB of disk space. However, due to key versioning and background compactions, the actual database size may be much bigger.

% If 50\% of the block contains popular objects (factor=1) when read into the cache, it will waste 50\% of the cache space. XXX Not sure to continue this sentence XXX and in the worse case (factor=3) ~80\%. Clearly, the more popular keys that are packed in a single SST block, the higher the cache efficiency. Existing LSM tree designs by default does not optimize for caching efficiency which can be critical for serving fast reads.

% Therefore, by packing blocks with objects that have similar popularity (\ie ``hot-cold’’ separation), there is the potential of improving the performance of an LSM tree even if all its data is sitting in homogeneous storage.



==> migration.tex <==
%-------------------------------------------------------------------------------
\section{Migration Evaluation}
\label{sec:mig-eval}
%-------------------------------------------------------------------------------

\subsection{Approximated Migration Metric}
\label{sec:mig-eval}
We divide the contiguous NVM key space into smaller key ranges based on the corresponding SSTable bounds on QLC.
To evaluate the effectiveness of our migration metric in Eq \ref{eq:migration}, we exhaustively search through all NVM key ranges and select the one with highest metric value. 
We name this strawman policy as \texttt{exhaustive} search policy. 

Computing the precise value of migration metric requires learning three important parameters about every candidate key range: $p$ - its percentage of popular keys, $N$ - the size ratio between the NVM key range and the overlapped SSTable, and $s$ - percentage of overlapping keys in the SSTable. 
$p$ can be calculated by iterating over the btree index to find all valid keys within the NVM key range and ask clock cache to check if they are popular or not. 
$N$ can be learned from system metadata on size. 
Finally, $s$ can be calculated by checking the existence of every NVM key using the SSTable's bloom filter.

One obvious disadvantage of this \texttt{precise\_M} metric is that it is both time-consuming and CPU intensive to compute.
For a large database with tens or hundreds of thousand SSTables, it will take a long time to select what to migrate and cost a lot of CPU resources.
This deviates from our goal of a fast and efficient migration. 
Instead, we propose a more realistic solution by approximating the precise metric and name it as \texttt{approx\_M} metric. 
It aims to achieve efficiency in three orthogonal axes: CPU, time, and QLC write amplification. 
We break the entire key space into fixed-size pieces, called Bucket, and keep track of some useful metadata per bucket.
Since the bounds of migration key ranges dynamically change over time, the main idea is to use overlapped buckets to approximate values of $p$, $N$, and $s$ of the interested NVM key range. 
The smaller the bucket size, the more precise our approximation can be. 
However, it is at the cost of keep more data in memory. 
A reasonable choice of bucket size is the average number of kv pairs in a SSTable on QLC.
In this work, we choose a bucket size of 64000 since most experiments use 64MB SSTable with an average item size of 1KB. 

Every Bucket contains 3 types of fields for its fixed-size key space: a counter that stores the number of unique keys present on NVM, a float that stores the ??? averaged overlap ratio of migration key ranges that overlaps with this key space, and a popularity bitmap. \todo{more to explain the details here} 


We introduce two additional migration metrics as baselines to compare. 
The \texttt{rand} metric assigns every candidate key range with a random value and picks the one with the highest value. 
It does not consider popularity or overlap ratio and ignores the possible effect of QLC write amplification. 
The \texttt{max\_unpop} metric ignores overlap ratio and only considers popularity. 
It picks the NVM key range with the highest number of unpopular keys. 
We choose YCSB-A, a write intensive workload, to analyze how do these four metrics perform along the axis of throughput, QLC write amplification and CPU utilization. 
Fig \ref{fig:mig-metric} and Table \ref{tab:mig-tput} summarizes the results. 
\begin{figure}[!t]
    \subfloat[]{
      \centering
      \includegraphics[width=0.8\columnwidth]{paper/figures/mig_metric.png}
      \label{fig:mig-metric}
    }
    \newline
    \subfloat[]{
      \centering
      \includegraphics[width=0.8\columnwidth]{paper/figures/mig_policy.png}
      \label{fig:mig-policy}
    }
    \caption{~\ref{fig:mig-metric} Comparison of different migration metrics under \texttt{exhaustive} search policy. ~\ref{fig:mig-policy} Comparison of different migration policies under \texttt{approx\_M} metric.}
    \label{fig:mig-eval}
\end{figure}



\begin{table}
    \centering
    \small 
    % \begin{tabular}{p{4cm}p{1.4cm}p{1.4cm}p{1.4cm}p{1.4cm}}
    \begin{tabular}{ |c | c | c | c|}\hline
      %\toprule 
      & \texttt{max\_unpop}  & \texttt{approx\_M} & \texttt{precise\_M} \\
      %\midrule
      \hline
      \texttt{rand-2} & 167.3 & 168.5 & 166.7 \\
      \hline
      \texttt{rand-4} & 176.0 & 176.9 & 173.8 \\
      \hline
      \texttt{rand-8} & 179.3 & 182.4 & 175.5 \\
      \hline
      \texttt{exhaustive} & 162.2 & 179.9 & 49.3 \\

      %\bottomrule
      \hline
    \end{tabular}
    \caption{Summary of throughput in (Kops/s) for different combinations of migration metrics and policies. Use YCSB-A workload: 50\%write-50\%reads, zipfian 0.8, 100 million key dataset, 1KB KV size, 100 million requests, 8 partitions, and 10 allocated CPUs.}
    \label{tab:mig-tput}
\end{table}

We find that while \texttt{precise\_M} metric has low QLC write IO, it almost doubles the CPU utilization compared to other metrics. 
This is because for every migration, it iterates over the btree index, uses clock cache for key popularity and bloom filters for key existence for all candiddate NVM key ranges that span across the entire key space of the partition. 
For this experiment where every partition owns around 210 SSTables, we observe an average migration time of 30 seconds. 
Since migration using \texttt{precise\_M} metric is too slow that it fails to capture its central role of garbage collection, \name has to aggressively rate-limit foreground client writes until migration frees enough space on NVM. 
This also translates to lower overall throughput of only 49.3 Kops/s, which is less than 1/3 of others' throughputs. 

On the other hand, \texttt{rand} metric runs fast, with an average migration time of 0.86 seconds. 
However, because its random nature makes it more likely to pick bad decisions, which on average moves only 12K items to QLC, it has to trigger a total of 1576 migration to free enough space, compared to ~516 migrations in other metrics. 
Thus, its total QLC write IO is very high, which is close to the size of the entire dataset. 

Both \texttt{max\_unpop} and \texttt{approx\_M} metrics achieve high throughputs, low QLC write IO and low CPU utilization.
We consider them as strong candidate metrics for efficient migrations. 
\texttt{max\_unpop} performs well in the YCSB workload because SSTables on QLC eventually will contain all keys from the dataset as the system reaches a steady state.
The overlap ratio starts to become irrelevant.
\texttt{max\_unpop} and \texttt{approx\_M} metric converge to the same objective which is to maximize the number of unpopular keys during migration. 
However, in real workloads with fresh inserts and deletes, overlap ratio plays a more active role and we believe \texttt{approx\_M} is the best metric to use. 


\subsection{Randomized Policy}
The straw-man \texttt{exhaustive} search policy has some obvious downside.
Since every migration needs to consider all NVM key ranges to finally decide what to migrate, it becomes quite in-practical for large real-world databases that can have  hundreds of thousand SSTables.
We need a more robust mechanism that can finish within almost constant time and also generate decent solutions. 
Inspired by the power of two choices, we use a random sampling process to select a subset of migration key ranges. 
The more random choices we consider, the closer we are to \texttt{exhaustive} policy. 
We name this randomized search mechanism as \texttt{rand-i} policy where $i$ is the number of random choices. 
Every migration randomly selects $i$ NVM key ranges as the candidate set of migration key ranges.

We experiment with 3 values of $i$: \texttt{rand-2}, \texttt{rand-4} and \texttt{rand-8}, and evaluate them with the best \texttt{approx\_M} metric under YCSB-A workload.
Fig \ref{fig:mig-metric} shows their respective throughputs and QLC write IOs. 
As the number of random choices increases, QLC write IOs gradually drops from 69.8GB to 50.9GB, getting closer to the smallest write IO cost of \texttt{exhaustive} policy. 
Simultaneously, throughput gradually climbs up because it can move enough colder keys to NVM while keeping QLC write amplification low. 
In fact, \texttt{rand-8} policy has a slightly higher throughput than \texttt{exhaustive} policy because it takes less time in selecting what to migrate and is faster in terms of garbage collection. 

The combination of \texttt{approx\_M} metric and \texttt{rand-8} policy gives the best performance result (shown in Table \ref{tab:mig-tput}).
Also, they help achieve fast and efficient migrations in \name while ensuring low QLC write amplification as well low CPU utilization. 
We believe they are robust in real-world settings where datasets are huge and workloads has other realistic characteristics (\eg fresh inserts and deletes) that are not captured by common benchmark workloads like YCSB. 
All experiments in this work, by default, use \texttt{approx\_M} metric and \texttt{rand-8} policy.






% \begin{figure}[!t]
% 	\centering
% 	\subfloat[]{
% 	\label{fig:mig-metric}
% 		\includegraphics[width=0.8\columnwidth]{paper/figures/mig_metric.png}
% 	}
% 	\newline
% 	\subfloat[]{
% 	\label{fig:mig-policy}
% 		\includegraphics[width=0.8\columnwidth]{paper/figures/mig_policy.png}
% 	}
% % 	\caption{
% % 	~\ref{fig:mig-eval} Distribution of reads across LSM levels (L0-L4), memtable (mt) and block cache (bc).}
% 	\label{fig:mig-eval1}
% \end{figure}
